Clustering-based Partitioning for Large Web Graphs

Graph partitioning plays a vital role in distributedlarge-scale web graph analytics, such as pagerank and labelpropagation. The quality and scalability of partitioning strategyhave a strong impact on such communication- and computation-intensive applications, since it drives the communication costand the workload balance among distributed computing nodes.Recently, the streaming model shows promise in optimizing graphpartitioning. However, existing streaming partitioning strategieseither lack of adequate quality or fall short in scaling with alarge number of partitions.In this work, we explore the property of web graph clusteringand propose a novel restreaming algorithm for vertex-cut parti-tioning. We investigate a series of techniques, which are pipelinedas three steps, streaming clustering, cluster partitioning, andpartition transformation. More, these techniques can be adaptedto a parallel mechanism for further acceleration of partitioning.Experiments on real datasets and real systems show that ouralgorithm outperforms state-of-the-art vertex-cut partitioningmethods in large-scale web graph processing. Surprisingly, theruntime cost of our method can be an order of magnitude lowerthan that of one-pass streaming partitioning algorithms, whenthe number of partitions is large.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> app.tex <==
\appendix
\label{app:partransform}

For each edge $e(u, v)$ in graph stream $G_S$, its partition choice is determined by the deployment of the clusters, to which its two vertices belong. If both partitions of $u$ and $v$ cannot accommodate $e$, $e$ will be assigned to a partition that has extra space to maintain the workload balance (lines 15-16). Otherwise, when both $u$ and $v$ are in the same partition, $e$ vertex will be assigned to $P_u$ (lines 18-19), for satisfying edge clustering rule, not so, the higher degree between $u$ and $v$ will be cut (lines 21-22) to reduce vertex replicas, for satisfying cluster splitting rule.


\begin{algorithm}[h]
    \footnotesize
    \caption{Partition Transformation}
    \label{alg:transform}
    \hspace*{\algorithmicindent} \textbf{Input} Cluster Partition Strategy $a^*$, Cluster Set $clu[]$, Vertex \\ \hspace*{\algorithmicindent} Degree $deg[]$, Load Balance Factor $\tau$ \\
    \hspace*{\algorithmicindent} \textbf{Output} Partition Result
    \begin{algorithmic}[1]
        \State Let $a_i$ be the partition choice of cluster $c_i$;
        \State Initialize the array of load, $L_{max}=\tau\frac{|E|}{k}$;
        \For{$e(u, v) \in G_S$}
            \State $c_u, c_v \gets clu[u]$, $clu[v]$;
            \State $p_u, p_v \gets a_u, a_v$;
            \If{$|p_u| \geq L_{max}$ \textbf{or} $|p_v| \geq L_{max}$}
                \If{$|p_u| < L_{max}$}
                    \State assign $e$ to $p_u$;
                    \State \textbf{continue};
                \EndIf
                \If{$|p_v| < L_{max}$}
                    \State assign $e$ to $p_v$;
                    \State \textbf{continue};
                \EndIf
                \For{$p_i \in P$}
                    \State assign $e$ to $p_i$ if $|p_i| < L_{max}$;  \hfill $\rhd$ Load Balance
                \EndFor
            \ElsIf{$p_u$ \textbf{equal} $p_v$}
                \State assign $e$ to $p_u$\;
            \Else
                \State assign $e$ to $p_{u}$ if $deg[v] > deg[u]$;
                \State assign $e$ to $p_{v}$ if $deg[u] > deg[v]$; \hfill $\rhd$ Reduce Replicas
            \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm} 

==> optimization.tex <==
\section{Parallelization}
\label{sec:parallel}

%%%%%%% xk Jan 27 del %%%%%%%%%%%%%%%%%
%We next show how to parallelize CLUSP and explain why CLUSP can perform best partition result without using any global state tables in BFS stream order. For random stream order, we also provied a parallel implementations, which needs an additional $O(|G_m|)$ space.

%%%%%%% xk Jan 27 add %%%%%%%%%%%%%%%%%
{\color{blue}
Ideally, the workload of distributed graph partitioning is decomposed into a set of independent subtasks running on separated distributed nodes and computation cores. Now, we introduce the parallelization mechanism.
%expected to run as a set of independent subtasks on different computation cores.
%Similar to \cite{petroni2015hdrf,tsourakakis2014fennel,restream,xie2014distributed,karypis1996parallel}, CLUGP can also run in parallel instances to speed up the partition phase without communication for only a small quality trade-off.
}
% However, there exist considerable correlations between subtasks, especially for the series of greedy and heuristic streaming partitioning algorithms \cite{petroni2015hdrf,mayer2018adwise,gonzalez2012powergraph}.
% These algorithms use local best partition choices of predecessors to guide the choice of successors, so that the global state of partition choice needs to be recorded and synchronized, which becomes a bottleneck incurring much thread conflicting and efficiency degrading.

% In this section, we study the parallel mechanism which gets rid of the bottleneck of global state maintenance.
%There are two levels of parallelization in the mechanism, namely inter- and intra-node parallelization.

\subsection{Parallelism Mechanism}

Our parallelism mechanism works as follows.
In all three steps, each distributed node reads the partial graphs and performs clustering, game processing, and transformation locally.
All distributed nodes run in parallel without inter- communication. Furthermore, in the game process, the clusters of each distributed node can be segmented as a series of batches, which can further be parallelized by multiple threads within the distributed node (Figure~\ref{fig:algorithm}).
In general, the parallel mechanism is on two levels,  \emph{inter}- and \emph{intra}-node parallelization.
%In the last step, each node loads the partial graph again and performs partition transformation, which is done in parallel.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figure/parallel.pdf}
%     \caption{parallel architecture}
%     \label{fig:parallel}
% \end{figure}

{
    \color{blue}
    The inter-node parallelization is enabled by the breadth-first streaming order. The partial graph loaded each distributed node can be regarded as a subgraph of the original graph. Since the subgraph of each node is loaded bf breadth-first order, we consider that subgraphs of different distributed nodes are mostly disjoint.

    The intra-node parallelization is enabled by Algorithm~\ref{alg:streaming-graph-cluster}, which preserves the graph locality, so that two clusters tend to be adjacent in the graph structure, if their cluster IDs are close. For example, as shown in Figure~\ref{fig:cluster-example} (b), if neighbors of vertex $v$ arrive in the BFS order, vertex $v_1$ stands out to form a new cluster $c_1$ with its neighbor, so that subgraphs of $c_1$ and $c_0$ are structurally adjacent. Based on the observation, we divide clusters {\color{red} of a distributed node} into batches according to cluster IDs, for parallelization. We recommend setting the batch size to a constant integer multiple of $k$, {\color{red} since the mismatch between the number of partitions, i.e., $k$, and the batch size can potentially cause partitioning imbalance}. The imbalance will expand the solution space of the cluster partitioning problem, thereby increasing the time cost of finding the Nash equilibrium. Notice that heuristic-based methods \cite{petroni2015hdrf,mayer2018adwise,gonzalez2012powergraph} focus on edge-level processing, which is insufficient for supervising partitioning, if without the support of global states. By contrast, the clustering results of CLUGP preserve structural modularity, provide more stable information for parallelization, and therefore isolate most, if not all, of the mutual influence between partitions. {\color{red} we go through this next Mon}
}

% The inter-node parallelization is enabled by Algorithm~\ref{alg:streaming-graph-cluster}, which takes BFS ordered streaming graph as inputs.
% Algorithm~\ref{alg:streaming-graph-cluster} preserves the graph locality, so that two clusters tend to be adjacent in the graph structure, if their cluster IDs are close. For example, as shown in Figure~\ref{fig:cluster-example} (b), if the neighbors of vertex $v$ arrive in BFS order, the vertex $v$ will be splitted out and form a new cluster $c_1$ with its neighbor (vertex 1), so that $c_1$ and $c_0$ are structurally adjacent.
% Notice that heuristic-based methods \cite{petroni2015hdrf,mayer2018adwise,gonzalez2012powergraph} focus on edge-level processing, which is insufficient for supervising partitioning, if without the support of global states.
% By contrast, the clustering results of CLUGP preserve structural modularity, provide more stable information for parallelization, and therefore isolate most, if not all, of the mutual influence between partitions.

% The intra-node parallelization is enabled by the randomness of batch selection within a distributed node.
% In addition, all clusters of a distributed node will be separated into a series of batches for parallelization.
% Notice that the size of clusters within a batch can be different.
% The mismatch between the number of partitions, i.e., $k$, and the batch size can potentially cause workload imbalance.
% We tackle the problem in three aspects. First, the clusters are mostly equal-sized, according the clustering process. Second, in the game process, the batch size is set as a constant integer multiple of $k$, so that the workload of distributed nodes can further be balanced during the independent processing.
% Third, the mismatch can also be alleviated by partitioning transformation, according to the fine-grained tuning of edge partitioning supervised by the load balance factor.

%The clusters of each batch can be viewed as the player set in a game process, where each cluster's partition choice is treated as a rational strategy and is made independently.
%The partition task of each batch can thus be accomplished by a thread.

\subsection{Analysis}

%\begin{theorem}
%    The CLUGP has $\Theta(|V|)$ memory cost and $\Theta(|E|)$ time cost.
%\end{theorem}

{
    \color{blue}

We next analysis the time complexity of CLUGP in a single node or in parallel distributed nodes, and show why time cost of CLUGP is bounded by I/O.

For a single distributed node, as stated above, CLUGP has three steps.
In the streaming clustering step, CLUGP needs to traverse the streaming edges once for clustering, so the time cost is $O(|E|)$. The memory cost of this step is $O(2|V|+m)$, because Algorithm~\ref{alg:streaming-graph-cluster} needs three arrays to record vertex degrees, cluster IDs, and cluster volumes, respectively. 
Since the time cost of modifying and querying three arrays is $O(1)$, so the time cost of this step is bounded by I/O. 
In the cluster partitioning step, according to Algorithm~\ref{alg:nash equilibrium}, the time cost for each round of finding Nash equilibrium is $\Theta(m)$, and the round complexity is far less than $|E|$ (shown in Section~\ref{sec:clusp algorithm}), so the total average time complexity of cluster partitioning step is $\Theta(|E|)$. Additionally, the space cost of step two is $O(m)$. Although the computation time cost if larger than the I/O time, we can use the intra-node parallel mechanism to speed up the partitioning process, so the time cost of this step can also be bounded by I/O with parallelization. For the third step, CLUGP traverses the edge stream to perform partition transformation that merely takes $O(k)$ memory space. To perform transformation, we only need to query the vertex-to-partition mapping table, and the operation only takes $O(1)$ time, so the time cost of this step is bounded by I/O. Overall, the CLUGP time cost is $\Theta(|E|)$ and the total memory cost is $\Theta(|V|)$.

For inter-node parallelization, the time complexity of each distributed node is $\Theta(\frac{|E|}{T})$ and the memory complexity of each node is $\Theta(|V|)$, where $T$ is the number of distributed nodes. For each node, it only needs to load $\frac{|E|}{T}$ edges at each step. The time complexity for the streaming clustering and partitioning transformation to process each edge is $O(1)$. The memory cost of streaming clustering is $O(2|V|)$. In the cluster partitioning step, based on Section~\ref{subsec:analysis}, the average time complexity can be approximated as $\Theta(|E_{b}^{avg}| * \frac{m}{batchsize \times threads\_num})$, where $|E_{b}^{avg}|$ is the average number of the intra-cluster edges in each batch. The memory cost of this step is $O(bathsize \times threads\_num)$, which is far less than $O(|V|)$. Overall, time complexity of each distributed node is $\Theta(\frac{|E|}{T})$ and memory complexity is $\Theta(|V|)$.

}
%%%%%%% xk Jan 27 del %%%%%%%%%%%%%%%%%
%For the heuristic based streaming partitioning algorithm \cite{petroni2015hdrf,mayer2018adwise,gonzalez2012powergraph}, it is hardly to perform algorithm in parallel since they need to maintain the global status table timely. When an edges is deployed to the partition, the algorithm need to store its choice to benefit successors in the stream which is the read-write intensive process. Therefore, how to weaken the connections between the partition choice on the stream is the key issue.

%In our implementation, we make the parallelism implemented on the cluster level not on the edge level. More over, our parallelization plan is made according to three properties: a)
%the streaming order is BFS; b) the BFS order ensures that when clusters are generated, clusters with consecutive ID are adjacent in structure (as shown in Algorithm~\ref{alg:streaming-graph-cluster}); c) the cluster structure is more stable compared with the edge, and the cluster contains more information than edge.

%The first property enables the feasibility of cluster-level parallelism. The second property implies that clusters with discontinuous ID are most likely not adjacent in structure. In other words, the mutual influence of partition choices on the stream can be weakened if we split the cluster partitioning task to different computing nodes in the sequence cluster ID order. The third fact shows the advantages of cluster-level parallelism. For the edge-level parallelism, without global status table, the information carried by an edge is obviously not enough to complete the part of the partition task. Conversly, the information carried by an cluster represents the sub-structure of the graph, which is important for the partition task. Our parallel architecture is shown in Fig~\ref{fig:parallel}.

%%%%%%%%%%%%%% xk Jan 27 %%%%%%%%%%%%%%%%%%%%%%
%For random stream order, we also provied a parallel implementations, which needs additional $O(|G_m|)$ space.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% For the random streaming order, we need $O(|G_m|)$ extra space to satisfy property b and property c. In the process of streaming cluster, we build up an adjacency list to store the connection between clusters. When performing clusters segmentation in second step, the cluster will be divided according to the depth-first traversal order of the adjacency list.







==> problem.tex <==
\section{Problem Definition}
\label{sec:problem}

Given a directed graph $G=(V,E)$, where $V$ is a finite set of vertices, and $E\subseteq V \times V$ is a set of edges, an vertex-cut partitioning algorithm assigns all graph edges $e \in E$ to a set of partitions $\mathcal{P}$. For a distributed system, each partition corresponds to a distributed machine/node. The vertices are not unique across partitions and are therefore replicated to several partitions. Therefore, the {\it replication factor} is considered as a general metric for measuring the partitioning quality so that the computation workload is balanced and the communication overhead is minimized.

Following the setting of \cite{BCSU3, zhu2016gemini,hua2019quasi}, we also suppose the edge stream of $G$ arrive in breadth-first (BFS) order, since most real web graphs are formulated and crawled in BFS order.

\begin{definition}[{Edge Streaming Graph Model}]
    The edge streaming graph model $G_S$ assumes edges of an input graph $G=(V,E)$ arrive in BFS order $\{e_1, e_2, \cdots, e_{|E|}\}$, where each edge $e_i=(u,v,w)$ indicates a directed edge form vertex $u$ to vertex $v$ with weight $w$.
\end{definition}

In vertex-cut streaming partitioning, partitioning algorithms perform single- or multi-pass over the graph stream and make partitioning decisions for computational load-balancing and communication minimization.

\begin{definition}[Vertex-Cut Streaming Partitioning Process]
    For each edge $e_i \in E$ arriving in the graph stream $G_S$, the vertex-cut streaming partition algorithm assigns it to partition $P_i \in \mathcal{P}$, such that $E_1\cup E_2\cup \cdots \cup E_k = E$ and $E_i \cap E_j = \emptyset$ ($i \neq j$).
\end{definition}

Formally, the goal of vertex-cut streaming partitioning is to minimize the replicate factor and the relative load balance. We follow the same definition of the partitioning goal used in \cite{gonzalez2012powergraph,petroni2015hdrf} as follows.
\begin{equation}
    \label{eq:metric}
    \begin{split}
        & minimize \frac{1}{|V|}\sum_{v\in V}|A(v)| \quad s.t. \frac{\max_{P\in \mathcal{P}}|P||\mathcal{P}|}{|E|} \leq \tau, P \in \mathcal{P} \\
    \end{split}
\end{equation}
where $|A(v)|$ is the number of partitions that hold vertex $v$ , $|P|$ denotes the number of edges in partition $P$, and $\tau \geq 1$ is a threshold for imbalance. By minimizing the replicate factor, the communication cost during graph computation is minimized, simultaneously.


\subsection{Web graph}
\label{subsec:Web graph}
In this subsection, we give a brief introduction about the property of web graph. According to Kumaret al. \cite{kumar1999trawling, kumar1999extracting} and Kleinberg et al.\cite{kleinberg1999web}, the degree distribution of the Web follows power law approximately.
\varGamma 





==> related work/crowdsourcing论文/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we study the problem of TCSC, which enables time-sharing collaboration among multiple workers towards long-term continuous spatial crowdsourcing applications. We propose an entropy-based quality metric for measuring the incompleteness of the crowdsourced results. Based on that, we study quality-aware task assignment algorithms with budget constraints for both single- and multi-task cases.
For the single-task case, we prove that the problem is NP-hard and devise algorithms with guaranteed approximation ratios. We further investigate novel indexing and pruning techniques for accelerating the process. For the multi-task case, we consider two variants, summation and minimum quality optimization with budget constraints. For both variants, we prove its NP-hardness and submodularity of quality functions, so that the framework of single-task case can be generalized and deployed. In particular, we design a parallel mechanism for accelerating the process of the summation quality optimization. Extensive experiments on real and synthetic dataset show that our proposals achieve good efficiency and scalability.

%considers tasks that take a long time to finish and involves time-sharing among multiple workers. We first assign tasks in the single-task scenario, and propose approximation algorithms and optimization strategies to enhance the efficiency of the single-task scenario. We further propose the task assignment of different variants in the multi-task scenario and design a parallel framework to deal with the problem of worker conflict among multi-tasks. We show through extensive experiments that our proposals are efficient. 

==> related work/crowdsourcing论文/experiment.tex <==
\section{Experiments}
\label{sec:experiments}

We cover the experimental setup in Section~\ref{subsec:setup}, and report the performance results of our proposals in Section~\ref{subsec:ret}.

\subsection{Experiment Setup}
\label{subsec:setup}

{\bfseries Dataset.}\footnote{Default parameters are bolded.}
We use a real dataset\footnote{ https://www.microsoft.com/en-us/research/publication/t-drive-trajectory-data-sample/} containing $10,357$ worker trajectories for representing workers' movements. For each worker trajectory, we randomly cut out a set of pieces, ranging from $1$ to $5$ time slots, as a worker's active slots.
%{\bf explain how the available slots are registered.}
We generate TCSC tasks' locations with Theodoridis et al.'s data generator\footnote{http://chorochronos.datastories.org/sites/default/files/algorithms\\/SpatialDataGenerator.zip} following {\bf uniform}, Gaussian, and Zipfian distributions.
We also use a Beijing POI dataset for representing tasks' locations\footnote{https://ieee-dataport.org/documents/beijing-poi-datasets-geographical-coordinates-and-ratings}. We set the cost for an assignment to be the distance that a worker moves to the assigned task, following the common setting of spatial crowdsourcing~\cite{todsurvey}\cite{tong17}.
We vary the number of TCSC tasks to test the scalability of our proposals by setting the number of tasks as 100, {\bf 300}, and 500, respectively.
For each TCSC task, we set the task length (i.e., the number of subtasks) to 300, {\bf 500}, and  1000, respectively.
The budget is set to $50$, {\bf 100}, $200$, corresponding to about 12.5\%, 25\%, and 50\% of the average cost of a TCSC task in the default setting. By default, $k$ is set to $3$ for the $k$-NN interpolation, $t_s$ is set to $4$. and the number of cores is set to $10$ for multi-task parallelization.
%as the 20\%, {\bf 30\%}, and 50\% of the total cost of the TCSC task.

%{\bfseries Task dataset.}
%We set the length of TCSC task as $300$, {\bf $500$}, and  $1000$.
%We use Theodoridis et al.'s data generator~\footnote{http://www.chorochronos.org/sites/default/files/algorithms\\/SpatialDataGenerator.zip} to obtain sets of 100K, {\bf 500K}, and 1M objects that are uniformly distributed in a 10K$\times$10K space.
%
%In order to better simulate the real scene, we consider the task assignment under different task distributions. Task locations are generated from Uniform distribution, Gaussian distribution or Zipf distribution within a rectangle of $100*80$ in the 2D coordinates. The start time and completion time of tasks are drawn from Uniform distribution. The implementation of task assignment under different distributions shows the scalability of our proposed strategy.

{\bf Competitors.} To our best knowledge, this is the first study on TCSC problem, so there is no existing baseline solutions.
To comprehensively evaluate our proposals, we consider two competitors for single TCSC task scenario, {\it Approx} and {\it Approx*}. The Approx solution is given by Algorithm~\ref{alg:single}, but without optimization techniques in Section~\ref{subsec:eff}. Approx* improves Approx by: 1) using tree-structured order-$k$ Voronoi diagrams to avoid redundant $k$-NN pre-computation; 2) using best-first searching and upper bound pruning for identifying the one with largest heuristic value.
Also, we consider three competitors for multiple TCSC task scenario: {\it Without Parallelization}, {\it Group-level Parallelization} and {\it Task-level Parallelization}, as introduced in Section~\ref{sec:multiple}.

{\bfseries Implementation.} All algorithms are implemented in Java and run a PC with Intel(R) Xeon(R) CPU $E5$-$2698v4$ @ $2.20$GHz and $256$GB main memory. By default, we use $12$ cores for running experiments on multi-task assignment.
Each reported value is the average of $20$ runs.
%We list the detailed setting of parameters in Table~\ref{tbl:para}.

%\begin{table}[!t]
%\small
%\centering
%\caption{Datasets}
%\label{tbl:para}
%\begin{tabular}{|c|l|}
%\hline
%Factor & Setting \\ \hline
%$m$ & 300, {\bfseries 500}, 1000\\
%\hline
%$|W|$ & 5000, 8000, {\bfseries 10000}\\
%\hline
%$\mathcal{T}|$ & 100, {\bfseries 300}, 500\\
%\hline
%$t_s$ & \\
%\hline
%$b$ & 20\%, {\bfseries 30\%}, 50\% \\
%\hline
%$k$ & 1, {\bfseries 3}, 5, 10 \\
%\hline
%\# of cores & 1, 2, 4, 8, 10, {\bfseries 12}, 14, 16 \\
%\hline
%distribution of task & {\bfseries uniform}, Gauss, Zipfian \\
%\hline
%\end{tabular}
%\end{table}

\subsection{Experiment Results}
\label{subsec:ret}


\begin{figure*}[!t]
\centering
\subfigure[Time of varying $m$] {\includegraphics[height=1in,width=1.7in]{exp/1-1.pdf}}
\subfigure[Time of varying $|W|$] {\includegraphics[height=1in,width=1.7in]{exp/1-2.pdf}}
\subfigure[Time of varying distribution] {\includegraphics[height=1in,width=1.7in]{exp/1-3.pdf}}
\subfigure[Time of varying $k$] {\includegraphics[height=1in,width=1.7in]{exp/1-4.pdf}}

\subfigure[Time Breakdown] {\includegraphics[height=1in,width=1.7in]{exp/2-1.pdf}}
\subfigure[Effect of $t_s$] {\includegraphics[height=1in,width=1.7in]{exp/2-4.pdf}}
\subfigure[Effect of Distributions] {\includegraphics[height=1in,width=1.7in]{exp/2-2.pdf}}
\subfigure[Effect of Budgets] {\includegraphics[height=1in,width=1.7in]{exp/2-3.pdf}}

\caption{Results of single-task assignment}
\label{fig:single-assignment}
\end{figure*}

%\begin{figure}
%  \centering
%  \includegraphics[width = 1.0\columnwidth]{exp/1-1.pdf}
%  \caption{Time of varying $m$  (sQM)}
%  \label{fig:single-m}
%\end{figure}

%We first present the results of single-task assignment with various parameters, and then show the performance of multiple task variants.

{\bfseries Single task assignment.}
We first test the efficiency of the two solutions, Approx and Approx*, by varying the number of time slots of a TCSC task. As shown in Fig.~\ref{fig:single-assignment} (a)
, Approx* improves over Approx by two orders of magnitude. As $m$ increases, the improvement is more significant. It is achieved by optimizing the approximation process with the tree-structured order-$k$ Voronoi diagram (Section~\ref{subsec:eff}).
%Fig.\ref{fig:single-assignment}(a) shows the results of vary the time slot $m$ of a task. As $m$ increases from 100 to 500, the running time of the assignment increases, because the approximation algorithm needs to complete more rounds, and the number of sub-tasks that can be selected for each round also increases.

%\begin{figure}
%  \centering
%  \includegraphics[width = 1.0\columnwidth]{exp/1-2.pdf}
%  \caption{Time of varying $|W|$  (sQM)}
%  \label{fig:single-w}
%\end{figure}
We test the effect of the number of workers in Fig.~\ref{fig:single-assignment} (b).
It can be observed that the time cost keeps stable and increases only slightly w.r.t. $|W|$.
The reasons are two-fold. First, the costs are calculated by travel distances between tasks and nearest workers according to the experiment setting. The increasing trend is moderate due to the good scalability of best-first NN searching algorithm adopted. Second, the slight increase shows that, with an increased number of workers, the completion ratios of tasks increase, resulting in higher costs. In all cases, Approx* outperforms Approx by at least two orders of magnitude.

%As $|W|$ increases, the total time cost is stable w.r.t.
%on finding nearest workers increases. The increasing trend is moderate due to the good scalability of the best-first searching algorithm. In all cases, Approx* outperforms Approx by at least two orders of magnitude.
%\begin{figure}
%  \centering
%  \includegraphics[width = 1.0\columnwidth]{exp/1-3.pdf}
%  \caption{Time of varying distributions  (sQM)}
%  \label{fig:single-distribution}
%\end{figure}
%\begin{figure}
%  \centering
%  \includegraphics[width = 1.0\columnwidth]{exp/1-4.pdf}
%  \caption{Time of varying $k$  (sQM)}
%  \label{fig:single-k}
%\end{figure}
We compare the two solutions by varying the distributions of TCSC tasks' locations in Fig.~\ref{fig:single-assignment} (c).
In all cases, the performance of Approx* dominates that of Approx by more than two orders of magnitude.
More, the time cost of Approx* remains relatively stable with different distributions, compared with the significant fluctuation of Approx.
We also test the effect of parameter $k$ for the data interpolation, in Fig.~\ref{fig:single-assignment} (d).
 The time cost increases w.r.t. the increase of $k$, since the cost of $k$-NN interpolation is higher for a larger $k$. The performance of Approx* dominates that of Approx.
%Two orders of magnitude better efficiency is achieved, compared with Approx.


To understand how the efficiency is achieved, we make detailed analysis in Fig.~\ref{fig:single-assignment} (e).
The improvements are in two parts. First, Approx* utilizes the implementation of the approximation of order-$k$ Voronoi diagram, and thus maximally reuses the computation of $k$-NN results. It can be observed that the cost of the interpolation (i.e., finding $k$ nearest subtasks) can be reduced by $4$ orders of magnitude.
Second, the tree-based pruning techniques can further reduce the cost of heuristic value calculation by more than an order of magnitude. This is consistent with our theoretical analysis in Section~\ref{subsec:eff}. Although Approx* incurs a little extra cost in building the tree-structure, the cost is well-spent given the remarkable efficiency gained.
We further examine the time cost spent on the tree-structure construction by varying parameter $t_s$, in Fig.~\ref{fig:single-assignment} (f).
 In all testing, the construction time is no more than $25$ ms, which is very efficient.
Also, the time decreases w.r.t. the increase of $t_s$, since a larger $t_s$ corresponds to a smaller number of tree nodes construction and therefore less construction time.


To examine the pruning effects of our proposal, we report the pruning ratios by varying the task length on different task distributions, as shown in Fig.~\ref{fig:single-assignment} (g).
The ratio is calculated by the dividing the number of slots executed with pruning techniques (Section~\ref{subsec:eff}) by the one without pruning.
It can be observed that our methods prune away more than 70\% subtask execution and therefore effectively accelerate the entire task processing. Similar trend is observed for the result on the real data.


We study the effect of budgets in Fig.~\ref{fig:single-assignment} (h).
 The time cost increases moderately w.r.t. $b$, since the number of executed subtasks also increases w.r.t. $b$.
Zipfian distribution has the lowest construction time. A task tends to incur higher cost under skewed distributions, so that
the number of executed subtasks is reduced and the corresponding time cost is less.

%In our setting, $b$ is defined according to percentage of executed subtasks.
%As a task with different distribution, the cost for completing a given percentage of subtasks varies widely. It may be the case that the tasks subject to the Gaussian distribution are concentrated in the areas with more available workers and therefore require the least budget, while the available workers are more discrete for the tasks subject to the Zipfian distribution and therefore require more cost....}




%
%
%The Fig.\ref{fig:single-assignment}(b) shows the results of varying the number of task. Clearly, as $|\mathcal{T}|$ increases, the running time of the assignment increases. The Fig. \ref{fig:single-assignment}(c) shows the results of varying the number of workers $W$. As $W$ increases, the running time of the assignment increases, because finding the nearest neighbor for each time segment is relative to the number of workers.  The Fig.\ref{fig:single-assignment}(d) shows the results under different distribution. Obviously, {\it Approximation*} performs more efficiently compared to {\it Approximation} in either distribution, and this results also verify the universality of our proposed method. The Fig.\ref{fig:single-assignment}(e) shows the results of varying $k$. As $k$ increases, the running time increases. In our work, we apply KNN to estimate the unprobed values. The larger k is, the more neighbors are needed, so the calculation will increase. Anyway, {\it Approximation*} is about 150 times faster than the baseline algorithm {\it Approximation} in all cases.
%
%Then, we shows the pruning ratio of {\it Approximation*} under different conditions. The Fig.\ref{fig:single-assignment}(f) shows the pruning ratio of varying $m$. As $m$ increases, the pruning ratio increases. As $m$ increases, the number of subtasks that can be selected per round increases, and the number of calculating heuristic values increases.
%
%The Fig.\ref{fig:single-assignment}(g) shows the pruning ratio of varying $b$. As $b$ increases, the pruning ratio increases. In our setting, $b$ is defined according to percentage of executed subtasks. As a task with different distribution, the cost for completing a given percentage of subtasks varies widely. It may be the case that the tasks subject to the gaussian distribution are concentrated in the areas with more available workers and therefore require the least budget, while the available workers are more discrete for the tasks subject to the zipf distribution and therefore require more cost.
%The Fig.\ref{fig:single-assignment}(h) shows the running time of each part of a task assignment process. We observe that the running time of {\it Approximation} is mainly in the part of calculating heuristic value, as it needs to finding the maximum heuristic value from all unexecuted subtasks at each round, and the calculation of a heuristic value refers to the summation of partial qualities of all slots. While {\it Approximation*} greatly avoids unnecessary computations, although it increases the overhead of the tree. But compared with {\it Approximation}, the efficiency of task assignment has improved significantly.

\begin{figure*}[!t]
\centering
\subfigure[Time w.r.t. number of cores] {\includegraphics[height=1in,width=1.7in]{exp/3-1.pdf}}
\subfigure[Time of varying distributions] {\includegraphics[height=1in,width=1.7in]{exp/3-2.pdf}}
\subfigure[Conflicts w.r.t. $|\mathcal{T}|$] {\includegraphics[height=1in,width=1.7in]{exp/4-1.pdf}}
\subfigure[Time of varying $|\mathcal{T}|$] {\includegraphics[height=1in,width=1.7in]{exp/3-3.pdf}}

\subfigure[Time w.r.t. number of cores] {\includegraphics[height=1in,width=1.7in]{exp/4-2.pdf}}
\subfigure[Time of varying $m$] {\includegraphics[height=1in,width=1.7in]{exp/4-3.pdf}}
\subfigure[Time of varying $|\mathcal{T} |$ (MMQM)] {\includegraphics[height=1in,width=1.7in]{exp/5-1.pdf}}
\subfigure[Time of varying $m$  (MMQM)] {\includegraphics[height=1in,width=1.7in]{exp/5-2.pdf}}
\vspace{-5pt}
\caption{Results of multi-task assignment}
\label{fig:multi-assignment}
\vspace{-10pt}
\end{figure*}


{\bfseries Multiple task assignment.}
We study the results on the summation quality case in Fig.~\ref{fig:multi-assignment} (a-f)
 and the results on the minimum quality case in Fig.~\ref{fig:multi-assignment} (g-h).

First, we compare the performance of the three competitors, group-based parallelization, task-based parallelization, and the basic solution without parallelization in Fig.~\ref{fig:multi-assignment} (a).
Both solutions with parallelization outperform the basic solution. Among the three, the task-based parallelization performs the best.
In particular, when the number of cores equals $10$, the task-based parallelization solution takes about two orders of magnitude less running time than the basic solution and the group-based parallelization solution, which is consistent with the analysis in Section~\ref{subsec:maxsum}.

We then compare the two parallelization methods by varying the tasks' distributions in Fig.~\ref{fig:multi-assignment} (b).
We can see that the Gaussian and Zipf distributions have higher costs. It is because that skewed datasets tend to incur larger numbers of worker conflicts.
Also, the number of worker conflicts increases with the number of tasks, as reported in Fig.~\ref{fig:multi-assignment} (c)
. Compared with group-based parallelization, the task-based parallelization saves orders of magnitude costs.

%As discussed earlier, we charge the independence of each task, and apply parallel technique to task assignment process to achieve better performance.The Fig.\ref{fig:multi-assignment_maxsum}(a) shows the results of varying cores. The main idea of Without-Parallelization is to treat all the tasks as a whole to allocate them, which does not involve parallel strategy. Therefore, changing cores has no impact on it.While for Group-level parallelization, the running time mainly depends on the size of a group. It can be seen that, while the size of each group is close, the running time decreases while cores increases, and it tends to be stable around 8. However, the whole algorithm will slow down due to the existence of a large group, in this condition, the running time of the entire algorithm is determined by the running time of the largest group, and changing cores may have no effect on the running time.
 %As for Task-level parallelization, increasing cores will decrease the running time, and it tends to be stable around 12.

%We can observe that the running time of Task-level parallelization is significantly less than Group-level parallelization under each distribution. When comparing different distributions, tasks with location satisfying the gaussian and zipf distribution take longer time to execute because there exists more worker conflicts compared to uniform distribution(as shown in the Fig.\ref{fig:multi-assignment_tasklevel}(a)). The worker conflicts will make the efficiency of task-level parallelization worse.

We report the scalability of our proposal w.r.t. the number of tasks in Fig.~\ref{fig:multi-assignment} (d)
. It can be observed that the task-based parallelization solution outperforms its competitor. When the number of tasks equals $300$, the task-based method takes about two orders of magnitude less time. More, the task-based parallelization method increases moderately w.r.t. the number of tasks, compared with the group-based method.

We then make more analysis with the task-based parallelization method. We test the effect of thread priority setting in Fig.~\ref{fig:multi-assignment} (e).
It can be observed that the priority adjustments for the threads accelerates the entire process.
In particular, when $16$ cores are used, about half of the cost can be saved. The reason is because the priority setting tends to revoke the thread resulting in the maximum heuristic value, and therefore breaks the tie of the blocked threads at an earlier stage.

We examine the performance of the algorithm by varying the parameter $m$, in Fig.~\ref{fig:multi-assignment} (f).
All methods increase moderately w.r.t. the increase of $m$.
In particular, Zipfian and Gaussian distributions take longer than the uniform case. The result is consistent with our analysis, because skewed task distributions have a larger chance for incurring worker conflicts, as reported in Fig.~\ref{fig:multi-assignment} (c).

%Then, we discuss the results of task-level parallelization. First, the Fig.\ref{fig:multi-assignment_tasklevel}(a) shows the number of worker conflicts when $|\mathcal{T}|$ increases. Clearly, the number of worker conflicts significant grows, especially for tasks with location satisfying the gaussian and zipf distribution. When the task location obeys the gaussian distribution, the distance between tasks is closer, and it is more likely to cause worker conflict. For tasks subject to zipf distribution, most of the tasks are distributed at the edge range, where the number of available workers is relatively small, so conflicts are more likely to occur.
%The Fig.\ref{fig:multi-assignment_tasklevel}(b) shows the performances with priory. If the priority is not used, the task with small heuristic value will also be executed, which wastes computing resources, and the computation time of rollback process will also be increased. Thus, the algorithm with priory is more efficient. Increasing cores will speed up the running time regardless of priority, and it tends to smooth around 12.
%The Fig.\ref{fig:multi-assignment_tasklevel}(c) shows the result of varying $m$. As $m$ increases, the running time also increases. Moreover, compared with uniform distribution, tasks subject to gauss or zipf distribution take longer to execute, because increasing $m$ brings about more worker conflicts.

We show the results on the minimum quality metric in Fig.~\ref{fig:multi-assignment} (g) and (h).
%For multiple-task assignment with max min quality metrics as the optimization target, we compare the performance of Approx and Approx* on in Fig.~\ref{fig:multi-assignment} (g) and (h).
First, we examine the time costs by varying $|\mathcal{T}|$ in Fig.~\ref{fig:multi-assignment} (g).
It can be observed that the time cost increases w.r.t. the increases of the number of tasks. The time costs for calculating the heuristic value is higher if the number of tasks is larger.
Second, we test the result by varying $m$ in Fig.~\ref{fig:multi-assignment} (h).
It can be observed that the running time increases as $m$ increases. %A larger $m$ corresponds to a TCSC task consisting of more subtasks, resulting in higher costs.
In both experiments, Approx* steadily outperforms Approx, demonstrating better scalability in terms of the number of tasks and subtasks.
%For example, when $|\mathcal{T}|=300$, Approx* is two orders of magnitude faster, as shown in Fig.~\ref{fig:multi-assignment} (g).

%In the end, we show the results of max min Quality. The Fig.\ref{fig:multi-assignment_maxmin}(a) shows the results of varying $|\mathcal{T}|$, as $|\mathcal{T}|$ increases, the running time will increase. Each round selects the task with the lowest task quality to complete one of the sub-tasks. The more the number of tasks, the more the number of times the task quality needs to be calculated, and the number of rounds of execution will also increase. We also compare the performance of {\it Approximation} and {\it Approximation*}, obviously, the efficiency of {\it Approximation*} is higher than {\it Approximation}.
% The Fig.\ref{fig:multi-assignment_maxmin}(b) shows the results of varying $m$, as $m$ increases, the running time will also increase. Since our budget is defined by the percentage of executed subtasks, the larger $m$ is, the more subtasks needs to be executed and the longer the running time.

%\begin{figure}[!t]
%\centering
%\subfigure[Time of varying $|\mathcal{T}|$] {\includegraphics[height=1in,width=1.7in]{exp/5-1.pdf}}
%\subfigure[Time of varying $m$] {\includegraphics[height=1in,width=1.7in]{exp/5-2.pdf}}
%\caption{Results of max min multi-task assignment}
%\label{fig:multi-assignment_maxmin}
%\end{figure}


%{\bfseries Scalability}: We show the results by increasing the number of tasks and workers at the same scale and compare the running time and memory costs.



==> related work/crowdsourcing论文/introduction.tex <==
\section{Introduction}
% no \IEEEPARstart
%spatial crowdsourcing
Spatial crowdsourcing or crowdsensing refers to harnessing human knowledge or sensors of participants' smart phones to retrieve qualitative or quantitative details related to physical locations of crowdsourced tasks.
For conventional spatial crowdsourcing, task assignment and fulfillment are often ``atomic'' in that either they are fully executed or not at all
 \cite{kazemi2012geocrowd,deng2013maximizing,cheng2015reliable,tong17,to2015server,DBLP:conf/icde/ChengLCS17,deng2015task,DBLP:journals/tetc/ZhangYLT19,DBLP:conf/icde/ChengLCS17,DBLP:conf/icde/ChenCZC19,cheng2016task,DBLP:conf/icde/ChengCY19}.
In this work, we consider a special type of spatial crowdsourcing, called {\it time-continuous spatial crowdsourcing} (TCSC {\it in short}).
TCSC is different, due to its temporal continuity, such that a spatial crowdsourced task takes long to finish, necessitating the time-sharing collaboration of multiple workers.
%We call this type of crowdsourcing {\it time-continuous spatial crowdsourcing} (TCSC {\it in short}), which
It finds broad applications in capturing the presence and duration of environmental features, e.g., air/water pollution monitoring\cite{DBLP:conf/iwqos/LiWZ19} and traffic surveillance\cite{DBLP:journals/sensors/ZhangZ0DG19}-\cite{DBLP:journals/wpc/SabirMS19}, which are prevalent in citizen science projects~\cite{citizenscience}.
%\footnote{https://www.nationalgeographic.org/encyclopedia/citizen-science/}.
%\footnote{http://www.gov.cn/gongbao/content/2019/content\_5363080.htm}.
%{https://www.epa.gov/air-research/community-air-monitoring-training}.

For example, in Fig.~\ref{fig:intro}, a crowdsourcer would like to monitor a set of selected sites for a period. Upon receiving the task, the TCSC server looks up the records of preregistered workers' spatiotemporal information. Indicating the undertaking of workers giving to the TCSC server, the registered spatiotemporal information consists of workers' available time slots, working regions, and so on, e.g., $\{ worker_1, \langle place~A, 1-2pm\rangle, \langle place~B, 7-8pm\rangle, \dots \}$. The task is then decomposed into a set of subtasks. Each subtask corresponds to a specific time slot and location. Subtasks are assigned to appropriate workers according to the assignment policy. Workers finish the assignment, e.g., probing environmental values, and send their results to the server. The crowdsourced results are aggregated and delivered to the crowdsourcer.

%time continuous task
%In such applications, crowdsourced tasks require continuously monitoring over a specified spatial unit. Air pollution levels are strongly correlated with local weather condition and nearby pollution emissions. air quality monitoring in citizen science.

\begin{figure}
\centering
\includegraphics[height=1.8in,width = 1\columnwidth]{fig/intronew.pdf}
\caption{General TCSC Framework}
\label{fig:intro}
\end{figure}

Quality is essential for such applications. It is infeasible to accomplish a crowdsourced task for all time slots, due to limited budgets and availability of workers. So, the probed data in crowdsourced results is inherently incomplete.
Interpolation (or extrapolation) alleviates the data incompletion problem by inferring unproved values with the probed ones.
However, the interpolation error may further affect the data precision, incurring the so-called data deficiency problem.
Ignorance of the facts of data incompletion and data imprecision would cause unreliable crowdsourced results.
Thus, it is of paramount importance to consider the data quality problem in the TCSC setting. To this end, we propose a general entropy-based metric for summarizing the amount of incompleteness and impreciseness of the crowdsourced results, which enables quality-aware TCSC assignment and balances the plannable expense and observable essence.

%to evaluate the quality of TCSC assignment, balancing the plannable expense and observable essence.

%The data deficiency problem can be alleviated by interpolating (or extrapolating) values of unprobed values from the probed ones. The idea is to estimate the unprobed values with the weighted average of probed values within a search neighborhood.
%In particular, inverse distance interpolation is believed to be the simplest and most popular interpolation technique \cite{li2004interpolation}\cite{gao2006voting} \cite{gao2006adaptive}.
%In this work, we aim to devise a solution bridging the gap between data interpolating and time-sliced data probing, rendering quality-aware TCSC crowdsourcing.

%The interpolation error for an estimated unprobed value is much dependent on the variance of neighboring probed values and corresponding distances.


There is a substantial difference between the TCSC problem and existing task assignment problems in spatial crowdsourcing. For example, existing works mostly focused on maximizing the total number of completed tasks~\cite{kazemi2012geocrowd}, on maximizing the number of performed tasks for an individual worker~\cite{deng2013maximizing}, or on maximizing the reliability-and-diversity score of assignments~\cite{cheng2015reliable}.
These solutions cannot be directly applied, as none of them look into the temporal continuous nature and corresponding quality issues of the TCSC problem.
To our best knowledge, we are the first to study the TCSC problem. %of time-continuous spatial crowdsourcing.

%In our work, we propose a metric for TCSC tasks, which is essentially an entropy function summarizing the amount of incompleteness and impreciseness of the crowdsourced results.

Nevertheless, the computational overhead of quality-aware TCSC assignment is high. Even a simplified version of the problem, i.e., single TCSC task assignment, is NP-hard, as shown in Section~\ref{sec:single}.
In this work, we study how the quality-aware TCSC assignment can be handled in an efficient and scalable way.
For task assignment policies, we consider both single- and multi-task scenarios. The single-task case is with the target of maximizing the task quality under budget constraints. We prove that the problem is NP-hard and further show that it can be approximated by a polynomial-time solution with guaranteed ratios. We also devise novel pruning and indexing techniques for the efficiency enhancement.
For the multi-task case, technical challenges lie on the correlations among tasks incurred by the conflicts during the worker selection, so that a trivial extension from the solution of single-task case is unapplicable. To tackle that, we devise a parallelization framework by distributing multiple correlated tasks onto independently running computation cores, so as to maximally utilize the independence between tasks.

The main contributions of this paper are as follows.

\begin{itemize}
\item We propose and formalize the novel TCSC problem.
\item We prove that the problem is NP-hard and therefore study approximation algorithms for accelerating the task assignment with quality guarantees, for both single- and multi-task scenarios.
\item We investigate novel indexing and pruning techniques for the efficiency of the single-task case.
\item We devise an efficient parallelization framework for the multi-task case, by breaking ties of correlated task groups with devised synchronization mechanisms.
\item We conduct extensive experiments on synthetic and real data to evaluate the efficiency and scalability.
\end{itemize}

%$Spatial\ crowdsourcing$ is the process of assigning a set of spatial tasks to a set of workers, which requires the workers to travel to the location of the spatial tasks. In traditional $spatial\ crowdsourcing$, spatial tasks and workers are atoms. A spatial task only needs to be assigned to one worker until the task is completed\cite{7}-\cite{10}. However, not all spatial task are as simple as these. In contrast, some spatial tasks often needs long time to perform, such as environment monitoring\cite{11}, traffic congestion detection\cite{12}. This type of tasks are impossible to be performed by one worker. Performing this type of tasks all the time needs enormous costs, while tasks often have limited costs. Inspired by the phenomenon of complex spatial tasks, in this paper, we will consider an important problem in the spatial crowdsourcing system, namely $spatiotemporal\ continuous\ crowdsourcing$, which assigns workers to spatial temporal continuous tasks. As far as we know, $spatiotemporal\ continuous\ crowdsourcing$ has not been addressed.

%In the sequel, we will illustrate the $spatiotemporal\ continuous$ $crowdsourcing$ by a motivation example of ... .

%Due to feature of the spatial temporal continuous task, these tasks may need more than one worker to preform. So we divide the task into multiple execution time slots and different time slots are performed by different workers. In this setting, there is often a $Budget$ constraint, for the total cost of the entire task. Thus, due to the limited task budget, it seems impossible to carry out the task all the time. More specific, the task may not be completely finished.

%%%%%%%%%%%%%%% quality by ting wang %%%%%%%%%%%%%%
%It is challenging to measure task finishing quality as each task has limited $Budget$ constraint. Task finishing quality is associated with the task completion ratio and task finishing distribution. When task completion ratio increases, task finishing quality increases. In particular, task finishing quality is greatest when task completion ratio equals 1(the task is finished completely). If two tasks have the same completion ratio, their task finishing quality will vary according to task finishing distribution. As shown in Fig.\ref{Example}, $task_1$ and $task_2$ complete three time slots. $task_1$ completes time slots $\left\{t_1,t_3,t_6\right\}$, while the executed time slots of $task_2$ mainly focus on the first half time. The executive condition of $task_2$ will cause results of the task is significantly affected if each value varies widely over time, then decreases the task finishing quality. Therefore, we want the task to be performed more often and uniform.
%
%%existing works fail
%Note that, existing works on $spatial\ crowdsourcing$ focused on assigning workers to tasks to maximize the total number of completed tasks \cite{7}, the number of performed tasks for a worker with an optimal schedule\cite{10}, or the reliability-and-diversity score of assignments\cite{9}. However, they did not take into account temporal continuous property of complex spatial tasks. Thus, we cannot directly apply prior solutions to solve the $spatiotemporal\ continuous\ crowdsourcing$.

%what we are to do
%In this paper, we first introduce the concept of $Quality$ denoting the task finishing quality to handle the challenge. Besides, we put forward single task assignment and its extension multiple task assignment based on the $spatiotemporal\ continuous\ crowdsourcing$. We also prove both kinds of task assignment are NP-hard, and thus they are very challenging to achieve the optimal solution.

%organization
The rest of this paper is organized as follows.
Section \ref{sec:preliminaries} introduces preliminaries, including concepts, quality metrics, and properties.
Section~\ref{sec:single} starts with the single-task assignment.
Section \ref{sec:multiple} extends the solution to the multi-task scenario.
Section \ref{sec:experiments} evaluates our proposals with extensive experiments.
Section \ref{sec:related} presents related works.
Section \ref{sec:conclusion} concludes the paper.
Table~\ref{tab:notations} summarizes the symbols and notations used.

%\begin{figure}
%\centering
%\includegraphics[height=2.3cm, width=6.5cm]{fig/2.pdf}
%\caption{Different task finishing distribution}
%\label{Example}
%\end{figure}

\newcommand{\tabincell}[2]{
}

\begin{table}[h!]
\centering
\caption{Summary of Notations}
\label{tab:notations}
\begin{tabular}{|c|l|}
\hline
Symbol & Meaning \\ \hline\hline
$\mathcal{T} = \{ \tau_i \}$ & a set of tasks \\
\hline
$\tau_i = \{ \tau_i^{(j)}\}_{j = 1}^m$ & a set of $m$ subtasks of task $\tau_i$\\
\hline
$\tau_i^{(j)}$ & a subtask of $\tau_i$ at $j$-th time slot\\
\hline
$c(\tau)$ and $c(\tau^{(j)})$ & cost of task $\tau$ and subtask $\tau^{(j)}$ \\
\hline
$W = \{ w_i \}_{i = 1}^{n}$ & a set of $n$ workers \\
\hline
$w_i^{(j)}$ & worker $w_i$ at $j$-th time slot \\
\hline
$m$ & number of subtasks of a task \\
\hline
$n$ & number of workers \\
\hline
%$x$ & task assignment matrix\\
%\hline
%$c_{\tau_i,w_j}$ & the traveling cost from $w_j$ to $\tau_i$ \\
%\hline
%$|a,b|_e$ & Euclidean distance between $a$ and $b$ \\
%\hline
$|a,b|_i$ & distance in time between slots  $a$ and $b$\\
\hline
$q(.)$  & quality metric function \\
\hline
$p(.)$ & subtask finishing probability function \\
\hline
$\rho_{err}(.)$  & interpolation error ratio function\\
\hline
\end{tabular}
\end{table}


==> related work/crowdsourcing论文/multiple.tex <==
\section{MULTIPLE TASK ASSIGNMENT}
\label{sec:multiple}

In this section, we study the multi-task assignment scenario, by considering two variants regarding the settings of optimization targets.
The first variant evaluates the overall quality by the summation of qualities of individual tasks, that belong to the given task set.
The second variant improves the overall quality by reinforcing the ``weakest'' single task, i.e., maximizing the minimum single task quality.
Both variants are on improving the overall quality of the given set of tasks with budget constraints\footnote{A dual version of our problem can be minimizing the task costs with quality constraints. It can be handled with the primal-dual method~\cite{DBLP:conf/approx/ChekuriK04}, which reduces the problem to the one studied in this work.}.% The details are hence omitted due to page limits.
In particular, we use $q_{sum}$ and $q_{min}$ to represent the optimization target functions, respectively. %For each function, we study corresponding properties supporting the approximation algorithms.

\begin{figure*}[ht!]
  \centering
\includegraphics[height=1.1in,width = 2\columnwidth]{fig/group.pdf}
  \caption{Worker Conflicting and Group-level Parallelization: an example of considering travel distances between workers and subtasks as costs.}
  \label{fig:group}
\end{figure*}

\subsection{Maximizing Summation Quality}
\label{subsec:maxsum}

The first optimization target is on maximizing the summation quality of all tasks. The problem is formalized as below.

\begin{definition}
{\bf Summation Quality.} Given a set of tasks $\mathcal{T} = \{\tau_1, \tau_2, ...\}$, we define the summation quality as:

    \begin{equation}
    \label{eqn:Quality_M}
           q_{sum}(\mathcal{T})= \sum_{i=1}^{|\mathcal{T}|}q(\tau_i \big{|} \tau_i \in \mathcal{T})
    \end{equation}
\end{definition}

\begin{problem}
{\bf Multiple-task Summation Quality Maximization with Fixed Budgets (MSQM {\it in short}).} Given a set of tasks $\mathcal{T} = \{\tau_1, \tau_2, ...\}$, the MSQM problem is to find a task assignment $x_i$ for each task $\tau_i\in \mathcal{T}$, such that the summation quality is maximized, and the overall cost $\sum c(\tau_i)$ does not exceed the given budget $b$.

   \begin{equation}
     \begin{aligned}
       Maximize~~q_{sum}(\mathcal{T})\\
       subject~to~\sum_{i=1}^{|\mathcal{T}|} c(\tau_i) \leq b
     \end{aligned}
   \end{equation}
 \end{problem}

We can prove that the MSQM problem is NP-hard, by reducing it from the sQM problem, whose NP-hardness is proved by Lemma~\ref{lem:np}.
%specifying the subtasks to be executed and then reducing it from the generalized assignment problem (GAP), whose NP-hardness is proved by Fisher et al.\cite{fisher1986multiplier}.

%\begin{lemma}
%    The $MSQM$ problem is NP-hard.
%\end{lemma}

%\begin{proof}
%The sQM problem is NP-hard, and the MSQM problem can be reduced to the sQM problem, if we treat the set of multiple tasks as a whole task. Thus, the MSQM problem is NP-hard.
%\end{proof}




\begin{lemma}
$q_{sum}(.)$ is submodular and non-decreasing.
\end{lemma}

\begin{proof}
We have proved that $q(.)$ is non-decreasing and submodular, by Lemma~\ref{lem:q}. The summation function is known as both convex and concave.
The $q_{sum}(.)$ function is a composite function of a summation function and $q(.)$ function. So, the lemma is proved, according to Lemma~\ref{lem:double}.
%
%Let $S_1,S_2$ denote two sets of tasks in $\mathcal{T}$. We are to prove that $q_{sum}(S_1\cap S_2) + q_{sum}(S_1 \cup S_2) \leq q_{sum}(S_1)+q_{sum}(S_2)$.
%Suppose two sets of sub subtasks $\tau^{(1)} \S_1$ and $\tau^{(2)} \in S_2$.
%We can have $\tau^{(1)}$
%
%In order to prove function $q_{sum}$ is submodular, we analyse the executed subtask $x1^{(k)},x2^{(k)}$ for each task $\tau^{(k)}$,
%where $x1^{(k)} \in S1$ $, x2^{(k)}\in S2$, $\tau^{(k)} \in \mathcal{T}$.
%As the function $q(\tau)$ is submodular function, then for each task $\tau^{(k)} \in \mathcal{T}$, there exists $q(x1^{(k)}\cap x2^{(k)})+q(x1^{(k)}\cup x2^{(k)}) \leq q(x1^{(k)})+q(x2^{(k)})$.
%While $q_{sum}$ is the sum of all task quality, obviously, $q_{sum}(S1\cap S2)+q_{sum}(S1\cup S2) \leq q_{sum}(S1)+q_{sum}(S2)$.
%Hence, the $q_{sum}$ is submodular function.
\end{proof}

%\begin{lemma}
%The function $q_{sum}$ is monotonous and nonnegative.
%\end{lemma}
%
%\begin{proof}
%Let $S1,S2$ denote two kinds of task assignments in $\mathcal{T}$, $S1 \subseteq S2$. Clearly, the number of the executed subtasks of $S2$ is larger than $S1$. According to the Theorem \ref{the:q_mon}, the quality function $q(\tau)$ is monotonous, then for the executed subtask $x1,x2$ of each task, $q(x1) \leq q(x2)$, where $x1 \in S1$ and $x2 \in S2$. Hence, the submodular function $q_{sum}$ is monotonous.
%From the Theorem \ref{the:q_mon}, we have proven $q(\tau) \geq 0$, and $q_{sum}$ is the sum of task quality in $\mathcal{T}$, so the submodular function $q_{sum}$ is nonnegative.
%\end{proof}

Based on the properties of submodularity and non-decreasingness, the framework of single task assignment, i.e., Algorithm~\ref{alg:single}, can be applied for handling the multi-task assignment case. The heuristic value is set as the increase of the summation quality divided by the corresponding cost (of a tentatively selected subtask), following the same greedy strategy. Then, the algorithm is to iteratively retrieve a subtask from all given $|\mathcal{T}|$ tasks that maximizes the heuristic value, so that the solution space is $|\mathcal{T}|$ times the size of the single task case, making the algorithm scale quadratically with $|\mathcal{T}|$.
The time complexity is $O(|\mathcal{T}|^2mlog^3(m))$.
To improve the scalability, we aim to derive a parallelization framework for distributing the calculation workload onto multiple computation cores. Ideally, each task can be running independently on different cores, so that the time cost would be $\frac{|\mathcal{T}|}{\text{\# of cores}}$ times that of running a single task, assuming the value of $|\mathcal{T}|$ is larger than the number of cores. But, there occurs correlations between tasks, if two subtasks running on different cores ``compete'' for one worker at some time slot. It happens because it is possible that two subtasks choose the same worker with lowest costs for minimizing the budget decrement.
We call this {\it worker conflicting}, as exemplified in Fig.~\ref{fig:group} (a), where there are three tasks ($\tau_1$ to $\tau_3$) and two workers ($w_1$ and $w_2$). There exist conflicts between $\tau_2$ and $\tau_3$, since they both take $w_1$ as the worker with the lowest cost.
%Notice that a worker can be the nearest neighbor for multiple subtasks simultaneously.

{\bf Group-level Parallelization.} We can have a graph of independent groups, if taking each task as a node and drawing an edge between any two conflicted tasks. If a group of nodes do not have any connections with other groups, it is an independent group. The optimization process of such a group is independent of others and therefore independent groups can be run in parallel.
For example, in Fig.~\ref{fig:group} (a), tasks can be divided into two independent groups, $\{\tau_1\}$ and $\{\tau_2,\tau_3\}$, if any pair of tasks do not compete for workers with lowest costs.

Is it sufficient for considering the conflicts on the lowest costs for deriving the independent groups?
%using $1^{st}$ nearest neighbor queries to derive the independent groups?
The answer is NO. For example, in Fig.~\ref{fig:group} (b), $\tau_2$ and $\tau_3$ have conflicts on $w_1$, so $\tau_3$ opts for $w_2$, who ranks as the worker with the second lowest cost. Unfortunately, $\tau_3$ further have conflicts with $\tau_1$, which has $w_2$ as the worker with the lowest cost. In general, if two subtasks belonging to different tasks are to be executed, one of them has to choose a worker with the second lowest cost, or even the latter.

One may get the independence graph by gradually expanding the searching regions.
For example, assume costs are calculated by the travelling distances from workers to tasks~\cite{todsurvey}\cite{tong17}. Then, a subtask takes the nearest worker as the worker with the lowest cost. For a given task, we call the circle centered at the task's position with the distance between the task and its nearest neighbor as its $1$-NN bound.
The independence graph can be obtained by the following steps.
Initially, we draw $1$-NN bounds for each task, as shown in Fig.~\ref{fig:group} (c). An edge between $\tau_2$ and $\tau_3$ is added, since the two tasks share the same worker that causes conflicts. Next, we draw $2$-NN bounds for both $\tau_2$ and $\tau_3$, so that there exist enough workers for being assigned to the two conflicting tasks, as shown in Fig.~\ref{fig:group} (d).
However, it shows that another worker is within $\tau_1$'s $1$-NN bound and $\tau_3$'s $2$-NN bound, so the two tasks have conflicts and the edge between them is added.
After that, we draw $2$-NN bound for $\tau_1$ and $3$-NN bound for $\tau_3$, as shown in Fig.~\ref{fig:group} (e). In general, if a node of the independence graph is with degree $d$, the $\text{(d+1)}$-NN bound should be drawn. The process repeats until no conflicts are detected.
A drawback of the gradual expanding method is on incurring large groups and heavyweight computation tasks, deteriorating the parallelization performance.

%But we found that it is common to have large groups, which inevitably slow down the running time of the entire parallel framework. Therefore, we hope to assign tasks in parallel in a multi-task scenarios.

%\begin{figure}
%\centering
%\subfigure[]{\includegraphics[height=0.9in,width=1.4in]{fig/group-1.pdf}}
%\subfigure[]{\includegraphics[height=0.8in,width=1.5in]{fig/group-2.pdf}}
%\vspace{-5pt}
%\caption{Example of Worker Conflicting}
%\label{fig:conflicts}
%\end{figure}



%We explain the worker conflicts among multi-task through some examples: task $\tau_2$ and task $\tau_3$ have worker conflicts as they have the same $1$-NN worker $w_1$ at a time slot, and $w_2$ is the nearest worker of task $\tau_1$. Then, the three task can be divided into two group(as shown in Fig \ref{conflicts}(a)). Meanwhile, $w_2$ is the $2$-NN of task $\tau_3$. If we assign worker $w_1$ to task $\tau_2$, then the task $\tau_3$ needs to be assigned to the $2$-NN worker $w_1$, and task $\tau_1$ and $\tau_3$ have worker conflicts, as shown in Fig \ref{conflicts}(c). Thus, the three task should be divided into a group. Tasks can be divided into groups only if the $k$-NN neighbour of task have no overlaps, as shown in Fig \ref{conflicts}(d).

%\subsubsection{Parallel Framework}
%
%{\bf We use an example to explain the worker conflicts.}

%Since there may be worker conflicts under multi-task assignment, multi-task assignment cannot be handled independently. The most straightforward way to assign multi-tasks is to treat all tasks as a whole and complete the task assignment as a single task(denoted as without parallelization). However, the computational cost is very high, as for each iteration, the approximation needs to select the highest heuristic value among all tasks until reaching the given budget. In order to allocate multi-tasks more efficiently, we devise specified parallelization framework by maximally utilizing the independence between tasks.

%Due to worker conflict, we are forced to assign tasks as a whole, but in fact, not all tasks have worker conflict with each other, and task conflict can be obtained in advance according to the nearest neighbor of subtasks. Therefore, we hope to divide the tasks into groups to ensure that there is no worker conflict among the tasks within the group. Then, tasks in each group are allocated in parallel(denotes as Group-level Parallelization). Compared with the without parallelization method, the group-level parallelization improves the efficiency of multi-task assignment, because the number of tasks in each group is far less than the total number of tasks. But we found that it is common to have large groups, which inevitably slow down the running time of the entire parallel framework. Therefore, we hope to assign tasks in parallel in a multi-task scenarios.

{\bf Task-level Parallelization.}
Hereby, we devise the task-level parallelization framework, as depicted in Fig.~\ref{fig:parallel}. We set a thread pool, with a master thread and a set of worker threads waiting for tasks to be concurrently executed.
The master thread is for maintaining the thread pooling on heartbeat monitoring, conflicting controlling, scheduling, and logging. To support the functionalities of the master thread, there are several associated data structures, {\it Heartbeat Table}, {\it Conflicting Table}, and {\it Logging Table}.

\begin{figure}[ht]
\center
\hspace{-20pt}\includegraphics[height=1.7in,width = 1\columnwidth]{fig/parallel.pdf}

  \caption{Task-level Parallelization: \textcircled{1} Periodically Sending Heartbeats to Master Thread; \textcircled{2} Reporting to Master Thread that Conflicts Detected; \textcircled{3} Looking Up Conflicting Table and Heartbeat Table, then Ask Worker Thread to Continue or Suspend; \textcircled{4} Adjusting Priorities of Worker Threads.}

  \label{fig:parallel}
\end{figure}

The Heartbeat Table stores periodically reported heuristic values from currently executed tasks. The scheduling algorithm sets priorities in accordance with the heuristic values of worker threads, so that the tasks with higher heuristic values are more likely to be processed. This is consistent with the greedy strategy of Algorithm~\ref{alg:single}. The priorities of worker threads are initialized as infinity in order to avoid thread starvation. Another purpose of monitoring the heartbeats is to record the execution progress, i.e., current heuristic values for tasks, so as to detect whether the given budget is met.

The Logging Table traces the historical records of the Heartbeat table. In the parallel environment, it is hard to strictly control the stopping condition, i.e., the timeline when the given budget is exhausted. It is unavoidable that threads with lower heuristic values are executed earlier than those with higher values, although such issues can be much alleviated with our priority settings.
Then, the logged information enables rolling back to the same stopping state for serialized task execution (e.g., Algorithm~\ref{alg:single}). This way, the task assignment plan derived by parallel methods is consistent with the non-parallel plan.

Last but not the least, the Conflicting Table stores a series of records for breaking the ties of conflicts. Assume three tasks, $\tau_1$, $\tau_2$, and $\tau_3$, are conflicted at time slot $t$. The information, including the conflicting task sets and corresponding conflicting time slot, is stored at the Conflicting Table of the master thread. In this example, a tuple $\langle \{\tau_1,\tau_2,\tau_3\}, t, 1 \rangle$ is recorded in the conflicting table.
Here, $1$ means the three tasks are to compete for the worker with the lowest cost.
Then, during the task processing, if $\tau_1$ is to execute conflicting slot $t$, its associated thread sends a message to inform the master thread. Upon receiving the message, the master thread looks up the Conflicting table and the Heartbeat table to retrieve the current heuristic values of $\tau_1$, $\tau_2$, and $\tau_3$.
If $\tau_1$'s current heuristic value is higher than $\tau_2$ and $\tau_3$, it continues with the execution of slot $t$. Meanwhile, the master thread checks the availability of workers and updates the record on the conflicting table, by changing the field ``{\it k-th NN}'' from $1$ to $2$, so that $\tau_2$ and $\tau_3$ would compete for the worker with the $2^{nd}$ lowest cost next time, because the first one has been taken by $\tau_1$.
If the heuristic value of $\tau_1$ is not the highest, $\tau_1$ is suspended.
The process continues until the given budget is exhausted.

%Challenges arise for task-level parallelization. First, how to deal with the problem of worker conflicting? Second, how to ensure that tasks with high heuristic values are completed first. To solve these problem, we design a parallel framework(denotes as task-level parallelization). Briefly, the parallel framework works as follows. At first, each task maintains a worker conflicting list. The master reads tasks and assigns a process to each task. Then, each task completes its assignment with the approximation algorithm. The process will be blocked if satisfy the following conditions:



%\begin{itemize}
%\item Condition 1: If the task meets time slot within the conflict list, the corresponding process is blocked and waits to wake up.
%\item Condition 2: If a task has been assigned $s$ time slots, the corresponding process is blocked and exchange information with the master.
%\end{itemize}
%
%
%When Condition 1 happens, it means that a worker conflict may occur at this time, then the blocked process sends message to the master to tell the master that "I" am blocked and passes the heuristic value back to the master. The purpose of condition 2 is to feed back heuristic value to the master, and determining the priority of the process based on the heuristic values. When the master has obtained all information, it will check if any processes can be awakened. Also, it is time to pass the rollback to the framework, if the cost is already over the given budget, then the parallel framework ends and the overbudget part of the assignment is deleted. We will call this a checkpoint. Basically communication between processors only occurs during these checkpoint moments.
%
%\begin{itemize}
%\item Checkpoint: All processes exchange its heuristic value with the master. The blocked processes due to condition 1, compare its heuristic value with other tasks. If there is a blocked process whose heuristic value is larger than any other process, the process can be awakened and the corresponding conflict removed from the conflicts list. If not, it continues to be blocked. As the blocked processes due to Condition 2, whether or not they can continue depends on the setting of their priority.
%
%\item Priority: According to the approximation algorithm, we needs to select the subtask which has the highest heuristic value. Thus, in order to save CPU computing resources, we set high priority on the process which has high heuristic value to reduce the computation of lower heuristic values. We can first compute the heuristic values of each task for the first iteration, and set the highest priory for the process with the highest heuristic value, on the contrary, set the lowest priory for the lowest process.
%
%    %how to define the function
%    The priory of other processes are set according to the blocked process(caused by Condition 1), as the blocked process can be awakened only if its heuristic value is higher than other processes. Thus, running processes with higher heuristic value as many as possible will make it faster for the blocked process to wake up. Here, we adopt several strategies and find the most suitable one.
%    \begin{itemize}
%    \item Default: Since no priority is set, all blocked processes by condition 2 can continue to execute. This method significantly increases the number of subtasks to be executed, which aggravates the rollback process.
%
%    \item Priory: Executing all blocked processes due to Condition 2 adds computational overhead, but there are some process should be performed (this processes may be executed in the following time, execution in advance can speed up the running time). Therefore, in order to be better in parallel, we choose to perform some of processes with high heuristic value, this ratio may be changed depending on the actual heuristic values.
%    \end{itemize}
%
%    \item Rollback: We try to save the execution of all the processes in the form of a log, and in the rollback process, the execution order is sorted according to the heuristic. Next, the execution is selected successively until meeting the given budget. The rollback process also ensures that the approximation algorithm selects the time slot with the maximum heuristic value to execute in each iteration.
%    \end{itemize}




\subsection{Maximizing Minimum Quality}
\label{subsec:maxmin}

The second optimization target is on maximizing the minimum quality of all tasks, so that the overall quality is optimized. The problem is formalized.
%\subsubsection{Problem Definition}
\begin{definition}
\label{def:Quality_{min}}
(Minimum Quality) Given a set of tasks $\mathcal{T} = \{\tau_1, \tau_2, \dots\}$, we define the minimum quality as:
    \begin{equation}
      q_{min}(\mathcal{T})= min \left\{q(\tau_i) \big{|} \tau_i \in \mathcal{T} \right\} %\nonumber
    \end{equation}
\end{definition}

\begin{problem}
    {\bf Multi-task Minimum Quality Maximization with Fixed Budgets (MMQM).} Given a set of tasks $\mathcal{T} = \{\tau_1, \tau_2, \dots\}$, the MMQM problem is to find a task assignment $x_i$ for each task $\tau_i \in \mathcal{T}$, such that the minimum quality is maximized, and the overall cost $\sum{c(\tau_i)}$ does not exceed the given budget $b$.
%    The fixed-budget maximum min quality problem is to find a task assignment $x_i$ for each task $\tau_i$ of multiple tasks $\mathcal{T}$ such that min task quality is maximized. Besides, the traveling cost of all tasks can not exceed the corresponding limited budget $b$:

       \begin{equation}
         \begin{aligned}
           Maximize~  &q_{min}(\mathcal{T})\\
           Subject~to~&\sum_{i=1}^{|\mathcal{T}|} c(\tau_i) \leq b  \\ \nonumber
         \end{aligned}
       \end{equation}
\end{problem}
\vspace{-20pt}

We can prove the NP-hardness of the MMQM problem by reducing it to the sQM problem. The submodularity and non-decreasingness of $q_{min}(.)$ function can be proved by Lemma~\ref{lem:qmin}. Hence, the $(1-1/\sqrt{e})$ approximation ratio of $q_{min}$ is achieved by iteratively executing the selected subtask from the task yielding the minimum quality. The subtask execution follows the framework of Algorithm~\ref{alg:single}.
To fast retrieve the task with minimum quality, we maintain a heap for $\mathcal{T}$ tasks. Notice that there is no worker conflict issues for the MMQM problem, since the subtasks are executed in a sequence. So, the total time complexity is $O(mlog^3(m)log(|\mathcal{T}|))$.

%The NP-hardness of the MMQM problem can be proved in a similar way of the MSQM problem, and is hence omitted due to page limits. Also, we can prove the submodularity of $q_{min}(.)$ function, as shown in Lemma~\ref{lem:qmin}.  Therefore, the framework of Algorithm~\ref{alg:single} can be applied for each task $\tau \in \mathcal{T}$.

%\subsubsection{Properties}
\begin{lemma}
\label{lem:qmin}
    $q_{min}(\mathcal{T})$ is submodular and non-decreasing.
\end{lemma}

\begin{proof}
We have proved that $q(.)$ is non-decreasing and submodular, by Lemma~\ref{lem:q}. The minimization function is known as a concave function.
The $q_{min}(.)$ function is a composite function of a minimization function and $q(.)$ function. So, the lemma is proved, according to Lemma~\ref{lem:double}.
\end{proof}


==> related work/crowdsourcing论文/new.tex <==
{\bf Quality Metric.} For condition 1), we define the concept of {\it subtask probability(reliability)}, based on the confidence of worker and the calculation of potential interpolation errors. For condition 2), we utilize an entropy function that returns a real-valued score for conveniently indicating the amount of inaccuracies in accordance with specific assignment strategies, as shown below.

\begin{definition}
({\bf Task Quality.}) Let $\tau$ be a task consisting of $m$ subtasks, $\tau = \{\tau^{(j)}\}_{1 \leq j \leq m}$. Each subtask $\tau^{(j)}$ is associated with a probability $p^{(j)}$. The quality of $\tau$, denoted by $q(\tau)$, is:

\begin{equation}
    \label{eqn:quality}
    q(\tau) = -\sum_{j=1}^{m}p^{(j)}\log_2\big{(} p^{(j)}\big{)}
    \end{equation}
\end{definition}

Next, we introduce the probability $p^{(j)}$ for subtask $\tau^{(j)}$, that serves as building blocks for the quality metric.

{\bf Subtask Probability.} The finishing probability of a TCSC task equals $1$, if all its subtasks are done, in correspondence to an ideal case that all subtasks are executed.
In practice, for a task consisting of $m$ equally sized  time slots, the finishing probability $p^{(j)}$ for each subtask $\tau^{(j)}$ is at most $\frac{1}{m}$. However, each worker is associated with a confidence, which is the probability (or
reliability) that the worker can successfully finish a task. Thus, the probability of the assigned subtasks is at most $\lambda\frac{1}{m}$.

For the probed subtask, the subtask probability concerns the interpolation errors. A common way of inferring a missing value from a discrete set of known values is known as inverse distance interpolation \cite{gao2006voting}\cite{gao2006adaptive}\cite{babak2009statistical}, which averages the values of its $k$ nearest neighbors, i.e., $k$ nearest subtasks on the timeline of a TCSC task.
Let $e$ be an executed subtask and $\tau^{(j)}$ be a subtask that is to be inferred. $|\tau^{(j)},e|_i$ denotes the distance in time between subtasks $\tau^{(j)}$ and $e$. Function $S_{kNN}(.)$ returns the set of $k$ executed subtasks with the smallest distances.

\begin{align}
\label{eqn:p}
p^{(j)} =
    \left\{
        \begin{array}{l}
        \lambda_{\tau^{(j)}} \frac{1}{m}\  if\ \tau^{(j)}\ is\ assigned \\
        \sum_{e \in S_{kNN}(\tau^{(j)})} \lambda_e \frac{1}{m} (1- \frac{|\tau^{(j)},e|_i}{k\cdot m}) if\ \tau^{(j)}\ is\ probed
        \end{array}
    \right.
\end{align}

$\lambda_e$ denotes the confidence of worker who is assigned to the subtask $e$. If there is no assigned subtask, then we define $|\tau^{(j)},e|_i$ equals $m$.

In summary, the concept of entropy is adopted to quantify the quality of crowdsourced results. The value of $q(\tau)$ ranges from $0$, i.e., the lowest information degrees (none of the subtasks are executed), to $log_2m$, i.e., the highest information degree (all subtasks are executed and all worker confidences equal $1$). 

==> related work/crowdsourcing论文/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

%We introduce key concepts in Section~\ref{subsec:basic}. We investigate the quality metric and its properties in Sections~\ref{subsec:quality} and \ref{subsec:property}, respectively.

In this section, we introduce basic concepts, propose the quality metric, and investigate its properties. For ease of presentation, we start with the single-task case (Sections~\ref{sec:preliminaries} and \ref{sec:single}), and extend it to the multi-task case (Section~\ref{sec:multiple}).

\subsection{Basic Concepts}
\label{subsec:basic}

\newtheorem{def1}{Definition}%[section]
%\begin{definition}
%\label{def:task}
{\bf A TCSC task and subtasks.}
%A spatiotemporal continuous task $\tau$ has its location $\tau_{loc}$ and the task completion time $\tau_t$; we divide the task completion time $\tau_t$ into $m$ time slots in order to make the subtask of a time slot can be completed by a worker. Clearly, the task $\tau$ is divided into $m$ subtasks $\left\{\tau_1, \tau_2, ..., \tau_m \right\}$, and we assume $f(\tau_i) =1$ if the subtask $\tau_i$ is accomplished, otherwise, $f(\tau_i) =0$. We use $\tau_e$ to denote the numbers of executed subtasks of task $\tau$.
A TCSC task $\tau$ has its location $\tau.loc$ and duration $\tau.dur$.
According to the batch size that tasks arrive in, the duration consists of at most $m$ equal-sized time slots. Thus, $\tau$ can be represented by a set of subtasks $\{\tau^{(j)}\}_{j = 1}^m$ such that each subtask $\tau^{(j)}$ takes $\tau.loc$ as its location, and the corresponding time slot as its duration. Formally, $\tau^{(j)}.loc = \tau.loc$ and $\tau^{(j)}.dur = \frac{\tau.dur}{m}$.
%\end{definition}

%\begin{definition}
%\label{def:worker}
{\bf Worker.} Let $W = \left\{ w_1, w_2, ..., w_n\right\}$ be a set of $n$ workers. Each worker is registered with a set of consecutive states to the SC server, indicating whether s/he is online for providing crowdsourcing services. A worker $w_i$'s state can be represented by a binary value $w_i^{(j)}$, indicating the availability of worker $w_i$ at time slot $t_j$.
In particular, $w_i^{(j)}$ equals 1, if $w_i$ is available for task assignment at time $t_j$; and equals $0$, otherwise.
%Let $W = \left\{ w_1, w_2, ..., w_n\right\}$ be the set of $n$ moving workers, and each worker $w_j$ has a trajectory which is uploaded before. The worker is in different positions at different time slots of a task. we use $\left\{w_j^{(1)}, w_j^{(2)}, ..., w_j^{(m)}\right\}$ to denote the location of the worker $w_j$ at each time slot of the task $\tau$. A worker $w_j^{(i)}$ at time slot $i$ can be in an either online or offline mode, and these two modes are arranged alternately. A worker is online when he is ready to accept tasks.
%\end{definition}
%}}

%\begin{definition}
%(Spatiotemporal Continuous Task Assignment)
{\bf Task Assignment.}
Task assignment is the mapping of workers to subtasks shown by a $n\times m$ matrix $x$, in which each element is a binary value $x_{i,j}$, representing whether worker $w_i$ is assigned to task $\tau$ at the $j$-th time slot.
$x_{i,j}$ equals $1$, if the assignment is made, and $0$ otherwise. In reality, the set of subtasks of a task can only be partially assigned, due to limited budgets and availability of workers. Also, an assignment is associated with a constraint $\sum_{i \leq n} x_{i, j} \leq 1$, meaning that each subtask can be assigned to at most one worker.
%\end{definition}

%%%          Commented by Xike 0604
%%{\bf Example.} Given a set of $4$ workers, $\{w_1, w_2, w_3, w_4\}$, and a TCSC task $\tau$ consisting of $6$ subtasks, $\{\tau^{(1)}, ..., \tau^{(6)}\}$, we show an example of task assignment in Figure~\ref{fig:assignment}. There are four assignment pairs $\langle\tau^{(1)}, w_1^{(1)}\rangle$, $\langle\tau^{(3)}, w_3^{(3)}\rangle$, $\langle\tau^{(4)}, w_2^{(4)}\rangle$, and $\langle\tau^{(6)}, w_4^{(6)}\rangle$, as shown in the bipartite graph in Figure~\ref{fig:assignment} (a).
%%An alternative representation of task assignment can be a binary matrix as shown in Figure~\ref{fig:assignment} (b), where a slash represents the unavailability of a worker at a given time slot. For each row, there can be at most one non-zero element, meaning that a subtask can only be assigned to one worker. The assignment strategy is on optimizing the corresponding cost, following the common settings of spatial crowdsourcing.
%%
%%\begin{figure}
%%\centering
%%\subfigure[Bipartite graph] {\includegraphics[height=1.3in,width=1.2in]{fig/assign_a.pdf}}
%%\subfigure[Matrix] {\includegraphics[height=1.3in,width=1.2in]{fig/assign_b.pdf}}
%%\caption{Task assignment}
%%\label{fig:assignment}
%%\end{figure}


%Let $W=\left\{ w_1,w_2,w_3,w_4\right\}$ denotes the set of available workers and $\tau = \left\{\tau_1,\tau_2,\tau_3,\tau_4,\tau_5,\tau_6\right\}$ denotes the set of subtasks of task $\tau$. In Figure~\ref{fig:assignment} (a), subtasks $\tau_1,\tau_3,\tau_4,\tau_6$ are executed, and the task assignment matrix $x$ is shown as Fig.\ref{assignment} (b). $\backslash$ indicates the corresponding worker is in offline mode, and he can not be assigned to perform subtask.
%}}

{\bf Cost.} The cost of a subtask $\tau^{(j)}$ is denoted as $c(\tau^{(j)})$. It can either be specified by workers or be calculated by the server, following the common setting of spatial crowdsourcing\footnote{If considering traveling distances as costs\cite{tong17}~\cite{todsurvey}, the nearest worker is usually selected in order to minimize the cost of taking a subtask. It is also possible to take the second nearest neighbor or the latter in multi-task scenarios, as covered by Section~\ref{sec:multiple}.}. Our work is general w.r.t. the type of cost.
The cost of a task is the summation of all its subtasks' costs, i.e., $c(\tau) =\sum^m_{j=1}c(\tau^{(j)})$.

%For an assigned worker-subtask pair $\langle \tau^{(j)},w_i^{(j)} \rangle$, we denote its cost as $c_{i,j}$, or equivalently the distance between $\tau^{(j)}$ and $w_i^{(j)}$. Then, total cost for a task assignment is the summation of travel distances for all subtask-worker pairs. Formally,
%\begin{equation}
%\label{equ:cost}
%C(x) %= \sum_{j=1}^{m}C(x_{\tau^{(j)}})
%= \sum_{j=1}^{m} \sum_{i=1}^{n} x_{i,j} \cdot c_{i,j}
%%x_{\tau^{(j)},w_i^{(j)}} c_{\tau^{(j)},w_i^{(j)}}
%\end{equation}


\subsection{Quality Metric}
\label{subsec:quality}

We define the metric for measuring the quality of a TCSC task, given the fact that a TCSC task cannot be fully assigned.
Therefore, there can be two possible states for a subtask, {\it executed} and {\it unexecuted}, corresponding to whether the subtask value is {\it probed} by assigned workers or {\it interpolated} by other probed subtasks. Initially, all subtasks are ``null''. If some subtasks are assigned and probed, their states are changed from ``unexecuted'' to ``executed''. Meanwhile, remaining unexecuted subtasks can be inferred from the executed subtasks by interpolation (or extrapolation).
%There can be three possible states for a subtask, {\it finished}, {\it interpolated}, and {\it null}. All states of subtasks are initialized as ``null''. With some ``null'' subtasks of a TCSC task being assigned, their states transform from ``null'' to ``finished''. Meanwhile, the remaining ``null'' subtasks can be interpolated or extrapolated by ``finished'' items.
So, the quality metric of a TCSC task should, 1) distinguish the quality between an probed item and an interpolated item; 2) be universal for covering the integrative action of different stated subtasks for the overall quality measurement.

{\bf Quality Metric.} For condition 1), we define the concept of {\it subtask finishing probability}, based on the calculation of potential interpolation errors. For condition 2), we utilize an entropy function that returns a real-valued score for conveniently indicating the amount of inaccuracies in accordance with specific assignment strategies, as shown below.

\begin{definition}
({\bf Task Quality.}) Let $\tau$ be a task consisting of $m$ subtasks, $\tau = \{\tau^{(j)}\}_{1 \leq j \leq m}$. Each subtask $\tau^{(j)}$ is associated with a finishing probability $p^{(j)}$. The quality of $\tau$, denoted by $q(\tau)$, is:

\begin{equation}
    \label{eqn:quality}
    q(\tau) = -\sum_{j=1}^{m}p^{(j)}\log_2\big{(} p^{(j)}\big{)}
    \end{equation}
\end{definition}

%Hereby, we propose a universal measure of task finishing quality for TCSC tasks. It is essentially an entropy function that returns a real-valued score for conveniently indicating the amount of inaccuracies in accordance to specific assignment strategies.

%It also enables efficiently quality-aware TCSC task assignment optimization, as will be shown in later sections.
%We first introduce the concept of {\it subtask finish probability} indicating the information degree of accomplishing a subtask. Based on that, we formulate the quality metric.

Next, we introduce the finishing probability $p^{(j)}$ for subtask $\tau^{(j)}$, that serves as building blocks for the quality metric.

{\bf Subtask Finishing Probability.} The finishing probability of a TCSC task equals $1$, if all its subtasks are done, in correspondence to an ideal case that all subtasks are executed.
In practice, for a task consisting of $m$ equally sized  time slots, the finishing probability $p^{(j)}$ for each subtask $\tau^{(j)}$ is at most $\frac{1}{m}$. Without losing generality, we can thus use an error ratio $\rho_{err}$ to measure the amount of information loss caused by interpolation errors.

\begin{align}
\label{eqn:p}
p^{(j)} = \frac{1}{m} (1 - \rho_{err}(\tau^{(j)}))
\end{align}
Accordingly, the probability $p^{(j)}$ equals $0$ for the ``null'' case, representing the zero knowledge about the subtask, and equals $\frac{1}{m}$ for the executed case, representing the total information gain of finishing the subtask.
Next, we show the calculation of error ratio $\rho_{err}$ for an interpolated subtask.
%For in-between values, i.e., $(0, \frac{1}{m})$, they can be taken for unfinished subtasks, indicating the amount of errors by interpolation or extrapolation.
%The overall information gain would be $1$, if all subtasks are finished.

%For unfinished subtasks, the results can be interpolated or extrapolated, if there exist some finished subtasks. Thus, its corresponding finishing probability lies within $[0, \frac{1}{m}]$.

{\bf Interpolation Error Ratio.}
A common way of inferring a missing value from a discrete set of known values is known as inverse distance interpolation \cite{gao2006voting}\cite{gao2006adaptive}\cite{babak2009statistical}, which averages the values of its $k$ nearest neighbors, i.e., $k$ nearest subtasks on the timeline of a TCSC task.%\footnote{We argue that our proposal can be general to other interpolation techniques, e.g., kriging, with slight modification to the information probabilities functions.}.

Intuitively, the error ratio is proportional to the distances between the interpolated value and its neighboring values~\cite{gao2006voting}\cite{gao2006adaptive}.
Let $e$ be an executed subtask and $\tau^{(j)}$ be a subtask that is to be inferred. $|\tau^{(j)},e|_i$ denotes the distance in time between subtasks $\tau^{(j)}$ and $e$. Function $S_{kNN}(.)$ returns the set of $k$ executed subtasks with the smallest distances. The equation of $\rho_{err}$ is as follows.
%Taking a numerical value interpolation as an example, the missing value can be inferred by averaging the values of $k$ nearest subtasks on the timeline of the task.
%Without losing generality, the finishing probability $p^{(j)}$ is formalized as:

\begin{align}
\label{eqn:rho}
\footnotesize
\rho_{err}(\tau^{(j)}) = \frac{\sum_{e \in S_{kNN}(\tau^{(j)})} |\tau^{(j)},e|_i}{k\cdot m}
\end{align}

%\begin{align}
%\label{eqn:rho}
%\footnotesize
%%\nonumber
%\rho_{err}(\tau^{(j)})\! =\!
%    \left\{
%        \begin{array}{l}
%        \! \frac{1}{k\cdot m}\sum_{e \in S_{kNN}(\tau^{(j)})}|\tau^{(j)},e|_i, ~~ if~|S_{kNN}(\tau^{(j)})| \geq k \\
%         \!(1-\frac{|S_{kNN}(\tau^{(j)})|}{k}) \! +\! \frac{1}{m}\sum_{e \in S_{kNN}(\tau^{(j)})}|\tau^{(j)},e|_i
%        \end{array}
%    \right.
%\end{align}

%The error ratio is thus proportional to the temporal distances between the interpolated subtask and neighboring subtasks, as shown below.
%Here, $|\tau^{(j)},e|_i$ denotes interpolation distance between subtask $\tau^{(j)}$ and one of its neighboring (finished) subtasks, $e$.
%The error would increase, if distance $|\tau^{(j)},e|_i$ increases. This is consistent with the fact that the error is proportional to the interpolation distances \cite{babak2009statistical}.

The value range of the error ratio $\rho_{err}$ is from $0$ to $1$. The error ratio equals $100\%$, if none of the subtasks of a task is executed. Accordingly, a lower error ratio value is achieved, if the target subtask has more proximate executed subtasks (i.e., smaller interpolation distances). For example, in Fig.~\ref{fig:voronoi}, $\tau^{(1)}$'s $2$-NN results are $\tau^{(2)}$ and $\tau^{(4)}$, whose distances from $\tau^{(1)}$ are $1$ and $3$, respectively. So, $\rho_{err}(\tau^{(1)})$ can be calculated as $\frac{1+3}{2*100} = 0.02$. Since $\tau^{(2)}$ is an executed subtask, its error ratio equals zero~\footnote{
It is possible that a subtask $\tau^{(j)}$ has less than $k$ nearest neighbors, e.g., at the starting stage of subtask assignment.
If $|S_{kNN}| < k$, we let $|\tau^{(j)},e|_i$ be $m$, indicating the largest possible interpolation distance.}.
Similarly, we can derive the error ratios and the subtask finishing probabilities for all the subtasks. Based on that, we can calculate the task quality, by Equation~\ref{eqn:quality}.

In summary, the concept of entropy is adopted to quantify the quality of crowdsourced results. The value of $q(\tau)$ ranges from $0$, i.e., the lowest information degrees (none of the subtasks are executed), to $log_2m$, i.e., the highest information degree (all subtasks are executed).

{\bf Extension for Worker Reliability.}
Our quality metric, i.e., Equation~\ref{eqn:quality}, is general in addressing the reliability of workers. We assume that each worker $w_i$ is associated with a confidence, represented by a probability $\lambda_i \in [0, 1]$ to indicate the reliability of $w_i$, following the setting of \cite{cheng2015reliable}.
Incorporating the reliability, the subtask finishing probability can be defined by both worker confidence and potential interpolation error. In particular, given subtask $e$, the finishing probability of an assigned task is $\frac{\lambda_e}{m}$, where $\lambda_e$ is the reliability of the worker assigned to subtask $e$.

Due to the incorporation of worker reliability, for an interpolated subtask $\tau^{(j)}$, the maximum finishing probability is no longer $\frac{1}{m}$, but the product of $\frac{1}{m}$ and the average of $\{\lambda_e\}_{e \in S_{kNN}(\tau^{(j)})}$. The extended form of subtask probability is as Equation~\ref{eqn:p2}.
\begin{align}
\label{eqn:p2}
p^{(j)} = \frac{1}{m} \cdot [\frac{\sum_{e \in S_{kNN}(\tau^{(j)})} \lambda_e}{k}  -
\rho_{err}(\tau^{(j)})]
%   (1- \rho_{err}(\tau^{(j)}, e)
\end{align}
Accordingly, the error ratio is determined by the summation of interpolation distances weighted by the worker reliability $\lambda_e$ and then divided by $k\cdot m$, similar to Equation~\ref{eqn:rho2}. The extended form of error ratio is as Equation~\ref{eqn:rho2}.
\begin{align}
\label{eqn:rho2}
\footnotesize
\rho_{err}(\tau^{(j)}) = \frac{\sum_{e \in S_{kNN}(\tau^{(j)})} \lambda_e \cdot |\tau^{(j)},e|_i}{k\cdot m}
\end{align}
Notice that probability $p^{(j)}$ equals $0$, if $S_{kNN}(\tau^{(j)})$ is an empty set, meaning that null of subtasks are currently done.
The probability $p^{(j)}$ is $\frac{\lambda_{\tau^{(j)}}}{m}$, if $\tau^{(j)}$ is an executed subtask.
If $\tau^{(j)}$ is interpolated, and the reliability of each worker for executing $S_{kNN}(\tau^{(j)})$ equals $1$, Equation~\ref{eqn:rho2} degenerates into Equation~\ref{eqn:rho}.

%Given subtask $e$, the confidence of the worker that
%
%The quality metric is general for extending to other scenarios,
%
%%Each worker $w_i$ is associated with a confidence $\lambda_i \in [0,1]$, which indicates the reliability of the worker that can do the task.
%
%For condition 1), we define the concept of {\it subtask probability(reliability)}, based on the confidence of worker and the calculation of potential interpolation errors. For condition 2), we utilize an entropy function that returns a real-valued score for conveniently indicating the amount of inaccuracies in accordance with specific assignment strategies, as shown below.
%
%However, each worker is associated with a confidence, which is the probability (or
%reliability) that the worker can successfully finish a task. Thus, the probability of the assigned subtasks is at most $\lambda\frac{1}{m}$.





%$\lambda_e$ denotes the confidence of worker who is assigned to the subtask $e$. Function $S_{kNN}(.)$ returns the set of $k$ executed subtasks with the smallest distances. For the assigned subtasks, $S_{kNN}(.)$ is all in itself. Accordingly, the probability $p^{(j)}$ equals $0$ for the ``null'' case, representing the zero knowledge about the subtask, and equals $\lambda \frac{1}{m}$ for the executed case, representing the total information gain of finishing the subtask.
%Next, we show the calculation of error ratio $\rho_{err}$ for an interpolated subtask.


%{\color{red}{\bf Quality Metric.} For condition 1), we define the concept of {\it subtask probability(reliability)}, based on the confidence of worker and the calculation of potential interpolation errors. For condition 2), we utilize an entropy function that returns a real-valued score for conveniently indicating the amount of inaccuracies in accordance with specific assignment strategies, as shown below.
%
%\begin{definition}
%({\bf Task Quality.}) Let $\tau$ be a task consisting of $m$ subtasks, $\tau = \{\tau^{(j)}\}_{1 \leq j \leq m}$. Each subtask $\tau^{(j)}$ is associated with a probability $p^{(j)}$. The quality of $\tau$, denoted by $q(\tau)$, is:
%
%\begin{equation}
%    \label{eqn:quality}
%    q(\tau) = -\sum_{j=1}^{m}p^{(j)}\log_2\big{(} p^{(j)}\big{)}
%    \end{equation}
%\end{definition}
%
%Next, we introduce the probability $p^{(j)}$ for subtask $\tau^{(j)}$, that serves as building blocks for the quality metric.
%
%{\bf Subtask Probability.} The finishing probability of a TCSC task equals $1$, if all its subtasks are done, in correspondence to an ideal case that all subtasks are executed.
%In practice, for a task consisting of $m$ equally sized  time slots, the finishing probability $p^{(j)}$ for each subtask $\tau^{(j)}$ is at most $\frac{1}{m}$. However, each worker is associated with a confidence, which is the probability (or
%reliability) that the worker can successfully finish a task. Thus, the probability of the assigned subtasks is at most $\lambda\frac{1}{m}$.
%
%For the probed subtask, the subtask probability concerns the interpolation errors. A common way of inferring a missing value from a discrete set of known values is known as inverse distance interpolation \cite{gao2006voting}\cite{gao2006adaptive}\cite{babak2009statistical}, which averages the values of its $k$ nearest neighbors, i.e., $k$ nearest subtasks on the timeline of a TCSC task.
%Let $e$ be an executed subtask and $\tau^{(j)}$ be a subtask that is to be inferred. $|\tau^{(j)},e|_i$ denotes the distance in time between subtasks $\tau^{(j)}$ and $e$. Function $S_{kNN}(.)$ returns the set of $k$ executed subtasks with the smallest distances.
%
%\begin{align}
%\label{eqn:p}
%p^{(j)} =
%    \left\{
%        \begin{array}{l}
%        \lambda_{\tau^{(j)}} \frac{1}{m}\  if\ \tau^{(j)}\ is\ assigned \\
%        \sum_{e \in S_{kNN}(\tau^{(j)})} \lambda_e \frac{1}{m} (1- \frac{|\tau^{(j)},e|_i}{k\cdot m}) if\ \tau^{(j)}\ is\ probed
%        \end{array}
%    \right.
%\end{align}
%
%$\lambda_e$ denotes the confidence of worker who is assigned to the subtask $e$. If there is no assigned subtask, then we define $|\tau^{(j)},e|_i$ equals $m$.
%
%In summary, the concept of entropy is adopted to quantify the quality of crowdsourced results. The value of $q(\tau)$ ranges from $0$, i.e., the lowest information degrees (none of the subtasks are executed), to $log_2m$, i.e., the highest information degree (all subtasks are executed and all worker confidences equal $1$).}
%%%%%%%%%%%% xk commented 0525 %%%%%%%%%%%%%%%%%
%When $|\tau^{(j)},e|_i$ increases, the error of subtask $\tau^{(j)}$ will increase, then the contribution rate of subtask $\tau^{(j)}$ to task quality decreases, and the final task finishing quality will reduce. $S_{KNN}(\tau^{(j)})$ denotes the $k$ executed subtasks closed to the unexecuted subtask $\tau^{(j)}$. In particular, when the task has none executed subtasks, the error of the unexecuted subtask $error(\tau^{(j)})=km$, then $p^{(j)}=0$, and we assume $q(\tau)=0$.
%%If the numbers of executed subtasks $\tau_e$ is less than $k$, $S_{KNN}(\tau^{(j)})$ also denotes the $\tau_e$ executed subtasks.
%
%So, the summation of subtasks' probabilities must be no more than one, i.e., $\sum_{j=1}^m p^{(j)} \leq 1$.
%
%The concept of entropy is adopted here to quantify the quality of crowdsourced results. The value of $q(\tau)$ ranges from $0$, i.e., the lowest information degrees (none of the subtasks are executed), to $log_2m$, i.e., the highest information degree (all subtasks are executed).
%%We have given the formula of $Quality$ above, then we attend to prove $Quality$ could denotes the task finishing quality accurately.
%
%%\begin{figure}
%%\centering
%%\includegraphics[height=4.5cm, width=6cm]{fig/metric_show.pdf}
%%\caption{Subtask quality function graph}
%%\label{metric}
%%\end{figure}
%
%The task finishing quality is related to its completion ratio the distribution of finished time slots. The higher the completion ratio, the higher the task completion ratio and quality.
%{\bf Add an Example. The observations show that our metric captures the features of task finishing quality.
%Figure \ref{metric} shows the subtask finishing quality changes with $p^{(i)}$, When there are no completed time slice, the subtask finishing probability equals 0 and the subtask finishing quality also equals 0. When $k < m$, through formula \ref{equ:pj}, subtask finishing probability varies greatly and subtask finishing quality increases greatly. When $k \geq m$, the inserting time slot either increases the subtask finishing probability slightly or does not change. Figure \ref{metric} clearly show these feature. To sum up, our metric captures the features of task finishing quality.}
%Also, a higher valued quality corresponds to a more uniform distribution. Therefore, our proof works in two cases. {\bf Let's keep the two cases at this moment.}
%
%Case 1 - the same task completion ratio :
%
%\begin{figure}
%\centering
%\includegraphics[height=5.5cm, width=6cm]{fig/1.pdf}
%\caption{Justification of $Quality$}
%\label{case1}
%\end{figure}
%
%Suppose we have a task $\tau_1$ and another task $\tau_2$ which have the same completion ratio, and its task completion distribution are as Fig.\ref{case1} (a).
%
%Assuming we use the 2 nearest executed subtasks to estimate the error of the unexecuted subtask, then for all unexecuted subtasks of $\tau_1$ and $\tau_2$, $\sum error(\tau^{(i)}_1) \leq \sum error(\tau^{(j)}_2)$, $\tau^{(i)}_1 \in \tau_1$ and  $\tau^{(j)}_2 \in \tau_2$. From the Formula \ref{equ:pj}, clearly, increasing the error of unexecuted subtasks will decrease the quality. Hence, In the case of the same task completion ratio, the higher the quality, the higher the task finishing quality.
%
%Case 2 - the same task completion distribution :
%
%Suppose we have a task $\tau_3$ and another task $\tau_4$ as Fig.\ref{case1} (b), and their task completion distribution are evenly.
%
%According to the Formula \ref{equ:pj}, $p^{(j)} = \frac{1}{m} (1 - error(\tau^{(j)})) <\frac{1}{m}$, if $\tau_i=0$. In short, the higher the completion ratio, the higher the quality. Hence, In the case of the same task completion distribution, the higher the quality, the higher the task finishing quality.


%----------------------------------------------
{\bf Summary.} We have shown the effectiveness of the metric in capturing the quality of various scenarios. In the sequel, we show two important properties of the metric, submodularity and non-decreasingness, enabling efficient task assignment algorithms with approximation guarantees.

\subsection{Properties}
\label{subsec:property}

%\subsubsection{Submodularity}
%Khuller et.al. \cite{article} proved a $(1-1/\sqrt{e})$ approximation guarantee for a modified Greedy algorithm under nonnegative submodular functions. In order to use the approximation algorithm,
We derive the properties of the task quality metric. We first recall the definition of submodular  functions.

\begin{definition}
\label{submodular}
({\bf Submodular Function \cite{cover2012elements}.}) Let $S$ be a finite set, and $2^S$ be the power set of $S$. A submodular function is a set function $f: 2^S \rightarrow \mathbb{R} $, if for any $X,Y\subset S$ satisfying $f(X\cap Y)+f(X\cup Y) \leq f(X)+f(Y)$.
\end{definition}

%Recall that we divide the task into $m$ subtasks, $S = \left\{ \tau^{(1)}1, \tau^{(2)},..., \tau^{(m)}\right\}$, so $S$ can be treated as a finite set, and our problem is to select a set of subtasks $X$ from $S$ to execute such that the task quality is maximized under a fixed budget, $X \subseteq S$. Here and in the following, we write $q(X)$ to denote the task finishing quality when executing the subtasks in the set $X$. As quality is similar to entropy \cite{cover2012elements}, it also satisfies the properties of entropy.

\begin{lemma}
\label{lem:double}
({\bf Composite Submodular Functions \cite{Lin}}.)
Assume a set $V$ and a function $h: 2^V \rightarrow \mathbb{R}$ that returns a real value for any subset $S \subseteq V$.
If $h$ is a non-decreasing submodular function and $\phi$ is a non-decreasing concave function $\phi: \mathbb{R} \rightarrow \mathbb{R}$, then function $\phi(h(S))$ is non-decreasing and submodular.
\end{lemma}

%\begin{lemma}
%\label{lem:submodular}
%The function $p^{j}$ is non-decreasing and submodular.
%\end{lemma}

\begin{lemma}
\label{lem:q}
Function $q(\tau)$ is non-decreasing and submodular.
\end{lemma}

\begin{proof}
The quality metric function $q(.)$ is a composite function of the entropy function and the finishing probability function, i.e., $p(.)$.
It can be proved that function p(.) is submodular and non-decreasing, as proved by Lemmas 7 and 8, in Appendix 8.1. More, the entropy function is known as non-decreasing and concave on the domain. According to Lemma~\ref{lem:double}, the quality metric function $q(.)$ is non-decreasing and submodular w.r.t. $\tau$.
\end{proof}

%\begin{lemma}
%\label{the:q_sub}
%The quality metric $q(\tau)$ is submodular.
%\end{lemma}
%\begin{proof}
%Let $\tau$ be a task containing a set of subtasks. Assume that $S_1$ and $S_2$ are two sets of subtasks of $\tau$.
%To show the metric $q(\tau)$ is submodular, it is sufficient to show that $q(S_1\cup S_2) + q(S_1\cap S_2)\leq q(S_1)+q(S_2)$.
%
%Without loosing generality, we define three disjoint sets $X_1$, $X_2$, and $X_3$, such that $X_1 = S_1 - S_2$, $X_2= S_1 \cap S_2$, and $X_3 = S_2 - S_1$. Then, it is equivalent to show that $q(X_1, X_2, X_3) +q(X_2)\leq q(X_1, X_2)+q(X_2, X_3)$.
%
%Let $p^{(j)}$ be the finishing probability of subtask $\tau^{(j)}$, and $\rho_2$ be the interpolation error ratio of
%
%%Let $x_1$, $x_2$, and $x_3$ be three elements of the three sets $\{S_1 - S_2\}$, $\{S_1 \cap S_2\}$, and $\{S_2 - S_1\}$, respectively.
%%We proceed to prove the submodularity of $q(\tau)$ with a simple chain rule.
%Then, to show the metric $q(\tau)$ is submodular, it is sufficient to prove:
%\begin{align}
%\nonumber q(S_1\cup S_2) + q(S_1\cap S_2)  & \leq q(S_1)+q(S_2) \\
%\nonumber q(X_1, X_2, X_3) +q(X_2)  & \leq q(X_1, X_2)+q(X_2, X_3)
%\end{align}
%
%
%
%Let $S1$ and $S2$ denote the subtask sets needed to be executed $S1,S2 \subseteq S$. Then, we use $x1,x2,x3$ to denote three different task assignment situations, $x1=S1-S2$ denotes executing the subtasks that belong to $S1$ and not to $S2$, $x2=S1\cap S2$ denotes executing the subtasks that belong to both $S1$ and $S2$, $x3=S2-S1$ denotes executing the subtasks that belong to $S2$ and not to $S1$. Then from a simple chain, we prove function $q(\tau)$ is submodular as follows:
%\begin{equation}
%    \begin{aligned}
%      & q(S1\cup S2) + q(S1\cap S2) \\
%      &= q(x1,x2,x3) +q(x2) \\
%                      &= q(x1,x3|x2)+2q(x2)   \\
%                      & \leq q(x1|x2)+q(x3|x2)+2q(x2) \\
%                      & \leq q(x1,x2)+q(x2,x3)  \\
%                      & \leq q(S1)+q(S2)  \\
%    \end{aligned}
%\end{equation}
%
%Where $q(x1|x2)$ denotes the quality increase when executing the subtasks in $x1$ based on the executed subtask set $x2$, and $q(x3|x2)$ in the same way.
%%Completing a new subtask will change the set $S_{KNN}$ of the unexecuted subtasks . For each subtask, the finishing probability is greater than or equal to the original value, so is the task quality. We will explain the reasons for the inequality as follows:
%From the Formula \ref{equ:pj}, we can get the finishing probability $p^{(j)} \leq \frac{1}{m} \leq \frac{1}{2} $ (assume $m \geq 2$). According to the properties of the function $xlogx$, the growth rate of the function decreases when increasing $x$, so the detailed proof of the inequality is as follows. Based on the subtask set $x2$ that has been executed, adding other execution sets $x1,x3$ will change the KNN sets before. We assume that the original error is $e$, the change of adding $x1$ to KNN value is $d1$, and the change of adding $x3$ to KNN value is $d3$. The inequality equivalently transform into
%
%$[(1-\frac{e-d1}{km})\frac{1}{m}]log[(1-\frac{e-d1}{km})\frac{1}{m}] + [(1-\frac{e-d3}{km})\frac{1}{m}]log[(1-\frac{e-d3}{km})\frac{1}{m}] - 2[(1-\frac{e}{km})\frac{1}{m}]log[(1-\frac{e}{km})\frac{1}{m}] $ $\geq [(1-\frac{e-d1-d3}{km})\frac{1}{m}]log[(1-\frac{e-d1-d3}{km})\frac{1}{m}] - [(1-\frac{e}{km})\frac{1}{m}]log[(1-\frac{e}{km})\frac{1}{m}]$.
%
%Simply, we use $w$ to denote $\frac{km-e}{km^2}$, and $v1, v3$ to denote $\frac{d1}{km^2}, \frac{d3}{km^2}$ then it becomes $(w+v1)log(w+v1)+(w+v3)log(w+v3)-2wlogw \geq (w+v1+v3)log(w+v1+v3) - wlogw$, and it is true as the derivative of the function $xlogx$ decreases.
%
%Hence, The function $q(\tau)$ satisfies the property of submodular, it is a submodular function.
%\end{proof}

%The submodularity captures the decreasing of marginal benefits.
The submodularity property captures the effect of marginal benefits decreasing in the measuring the TCSC quality. As the number of workers on finishing a task is increasing, the marginal value of adding a new worker is decreasing.
Also, the submodular property of the quality metric enables efficient optimization, e.g., submodular function maximization, where constant factor approximation algorithms are often available~\cite{article}. In the sequel, we discuss how the property is utilized and generalized for optimization problems in the TCSC task assignment applications.

%\begin{lemma}
%\label{the:q_mon}
%The submodular function $q(\tau)$ is monotonous and nonnegative.
%\end{lemma}
%
%\begin{proof}
%Let $S$ a sets of subtasks in $\tau$, and $e$ be a subtask of $\tau$ satisfying $e \notin S$. If we can show that the quality increases with executing $e$ based on $S$, i.e.,
%$q(S \cup e)  \geq q(S)$, then the function $q(\tau)$ is monotonous.
%
%Let us consider the quality change upon executing $e$ based on the execution of $S$. If none of the subtasks in $S$ is executed, the finishing probabilities change from zero to non-zero values, so that the quality value must increase.
%
%There are two possible states for subtasks of $S$, ``finished'' and ``interpolated''.
%
%According to Equation~\ref{eqn:p},
%
%According to Equation~\ref{eqn:p},
%
%Clearly, the number of the executed subtasks of $S2$ is larger than $S1$. According to the Formula \ref{equ:pj} from Section 3.2, the contribution rate of the executed subtask is greater than the unexecuted subtask. When the task continues to execute new subtask, the unexecuted subtask is either executed or the interpolation error of the subtask is reduced, both possibilities will increase the task finishing quality. Therefore, $q(S1) \leq q(S2)$, the submodular function $q(\tau)$ is monotonous.
%
%From the Formula \ref{equ:pj}, we can get the finishing probability $p^{(j)}$ within the range of $0$ and $\frac{1}{m}$, then $\log[ p^{(j)}] \leq 0$. Therefore, function $q(\tau) = -\sum_{j=1}^{m}p^{(j)}\log[ p^{(j)}] \geq 0$, and the submodular function $q(\tau)$ is nonnegative.
%
%\end{proof}






==> related work/crowdsourcing论文/related.tex <==
\section{Related Works}
\label{sec:related}

%There are many previous studies in spatial crowdsourcing, which requires workers traveling to locations of spatial tasks and performs tasks, such as taking photos/videos, repairing a house, and waiting in line at shopping malls. These works focused on assigning available workers to tasks with distinct goals, such as maximizing the number of assigned tasks\cite{kazemi2012geocrowd} \cite{to2015server}, minimizing the total cost of all workers \cite{deng2015task}, or maximizing the quality score \cite{cheng2015reliable} \cite{to2015server}.

There are many studies in spatial crowdsourcing, which requires workers traveling to locations of spatial tasks and performs tasks, such as taking photos/videos, repairing a house, and waiting in line at shopping malls. These works focused on assigning avaliable workers to tasks with distinct goals, such as maximizing the number of assigned tasks\cite{kazemi2012geocrowd} \cite{to2015server} \cite{DBLP:journals/pvldb/ChengJC18}, minimizing the total travel costs of all workers \cite{deng2015task} \cite{DBLP:journals/tetc/ZhangYLT19}, maximizing the quality score \cite{cheng2015reliable} \cite{to2015server} \cite{DBLP:journals/csur/DanielKCBA18}, maximizing quality task assignment by considering
both present and future workers/tasks \cite{DBLP:conf/icde/ChengLCS17},  or minimizing maximum delay of task assignment \cite{DBLP:conf/icde/ChenCZC19}.

Gummidi \cite{todsurvey} et al. categorize spatial tasks from two aspects, task complexity and the required number of workers. Regarding the task complexity, there are two types, atomic tasks and complex tasks, which depend on whether tasks can be divided into atomic subtasks. Atomic tasks are simple and only take one worker to complete \cite{kazemi2011privacy} \cite{cornelius2008anonysense}. On the contrary, complex tasks consists of at least two subtasks that need to be performed collaboratively. Complex tasks can be divided into atomic subtasks to be performed \cite{cheng2016task} \cite{benouaret2013answering}\cite{DBLP:conf/icde/ChengCY19}. For instance, \cite{cheng2016task} divides a spatial task according to the required worker skills, and assigned proper workers to each atomic tasks. %\cite{benouaret2013answering} considered the process of data collection, data selection, data assessment and proposed a location-based crowdsourcing framework to cope with these problems. %Our TCSC tasks belong to the complex tasks, but
However, previous works do not consider the task duration and the availability of workers, whereas a TCSC task often takes long to be completed by multiple workers.
%Our TCSC tasks belong to the complex tasks, while the difference from our work is that we consider a task takes a long time to complete. In our settings, there is only one task involved here.
%Due to the long task duration, a TCSC task needs to be divided into subtasks. As the tasks are defined differently, we cannot directly apply previous techniques to our problems.

Regarding the number of required workers, a spatial task can be assigned to either one or more workers. While assigning spatial tasks to multiple workers, the task quality can be improved by collecting more answers \cite{DBLP:conf/gis/KazemiSC13}. The similarity with our work is that both methods assign more than one worker to complete the task. The TCSC task quality is determined by the task finishing rates and distributions,%, and there is no situation where a subtask is performed by multiple workers at the same time.
while previous works on the task quality mostly focus on pre-task qualification test \cite{DBLP:journals/pvldb/LiuLOSWZ12}, or the assignment based on the expertise \cite{cheng2016task}, or abilities \cite{cheng2015reliable} \cite{DBLP:conf/gis/KazemiSC13} of the worker.

To summarize, a TCSC task belongs to the complex task type. It is of time continuous natures and quality concerns so that collaboration of multiple workers is needed. %the quality-aware task assignment requires multiple workers.
%belongs to the complex task and requires multiple workers. Also, we consider the time continuous nature and the quality of a task in the assignment.
Therefore, existing works cannot be directly applied to our problem.
%Therefore, we put forward a metric to measure the task quality and design approximation algorithms, pruning techniques, and parallelization methods for the task assignment optimization. %We assign tasks with a goal, that is, maximizing the task quality of assignments under the given budget. As the tasks are defined differently, we cannot directly apply previous techniques to tackle our problems. 

==> related work/crowdsourcing论文/single.tex <==
\section{SINGLE TASK ASSIGNMENT}
\label{sec:single}

We proceed to study the single TCSC task assignment problem.
In particular, we consider maximizing the quality of a single task with budget limits.
We prove that the problem is NP-hard.
For efficient task assignment, we devise heuristic algorithms that approximate the optimization targets in polynomial time with quality guarantees.
Nevertheless, we show that the polynomial solution incurs overheads unaffordable for the real-time task assignment scenarios.
Therefore, we propose novel indexing and pruning techniques to further enhance the task assignment efficiency.

We formalize and analyze the problem in Section~\ref{subsec:pdef}. We devise the approximation algorithm in Section~\ref{sec:single_alg}. We study efficient indexing and pruning techniques in Section~\ref{subsec:eff}.

\subsection{Problem Definition and Analysis}
\label{subsec:pdef}

\begin{problem}
{\bf Single-task Quality Maximization with Fixed Budgets (sQM {\it in short}).}
Given a TCSC task $\tau$ and a fixed budget $b$, the sQM problem is to find a task assignment matrix $x$, such that the quality $q(\tau)$ is maximized, and the cost $c(\tau)$ does not violate the given budget $b$.
\label{6}
\begin{align}
    Maximize~~ & q(\tau)  \nonumber \\
    %subject~~to~~ &\sum_{j=1}^{m} \sum_{i=1}^{n} x_{i, j}\cdot c_{i, j} \leq b  \nonumber
    subject~~to~~ &\sum_{j=1}^{m} c(\tau^{(j)}) \leq b \nonumber
 \end{align}

% \begin{align}
%    Minimize~~ &\sum_{j=1}^{m} c(\tau^{(j)})  \nonumber  \\
    %subject~~to~~ &\sum_{j=1}^{m} \sum_{i=1}^{n} x_{i, j}\cdot c_{i, j} \leq b  \nonumber
%    subject~~to~~ & q(\tau) \geq Q \nonumber
% \end{align}

\end{problem}

To solve the sQM problem is equivalent to evaluate a task assignment matrix yielding the maximum quality.
To give a sense of the size of the solution space, we assume a given set of $n$ workers and a task consisting of $m$ subtasks/timeslots. Thus, there could be an exponential number of possible worker-and-subtask assignment pairs $O(m^n)$.
Then, we prove that the $sQM$ problem is NP-hard, by Lemma~\ref{lem:np}.
%reducing it from another well-known NP-hard problem, $0$-$1$ Knapsack problem.

%\begin{definition}
%({\bf The 0-1 Knapsack Problem}~\cite{vazirani2013approximation}.) Given a maximum weight capacity $W$, and a set $C$ of objects, $C = \{a_i\}_{i=1}^{n}$, of which each object is with a weight $ws_i$ and a value $v_i$, the 0-1 Knapsack problem is to find a subset $C'$ ( $C' \subseteq C$) that maximizes $\sum_{a_i\in C'}v_i$ and satisfies $\sum_{a_i\in C'}ws_i \leq W$.
%\end{definition}

\begin{lemma}
\label{lem:np}
    The $sQM$ problem is NP-hard.
\end{lemma}

%\begin{lemma}
%    The $sQM$ problem is NP-hard.
%\end{lemma}

\begin{proof}
It is well known that maximizing a submodular function under a cardinality constraint (i.e., selecting at most $k$ elements) is NP-hard~\cite{Nemhauser1978}. If we consider the workers have unit cost, the budget constraint in our problem becomes the cardinality constraint. It has been proved in Lemma~\ref{lem:q} that the quality function $q(\tau)$ (i.e., the objective function to be maximized) is submodular, and thus a special case of our $sQM$ problem is also NP-hard.
\end{proof}

%\begin{proof}
%    For a given 0-1 knapsack problem, we can transform it to an instance of $sMQ$ as follows: In our problem, we divide the task $\tau$ into $m$ subtasks. Let $\tau = \left\{ \tau_i : i = 1, ..., m\right\}$ be the set of these subtasks, and $W =\left\{w_j : j = 1, ..., n \right\}$ be the set of workers, and each pair of subtask and worker $<\tau_i, w_j>$ denotes the corresponding $\tau_i$ is assigned to $w_j$. The the traveling cost $c_{\tau_i, w_j} = ws_i$ and the subtask quality $q_{\tau_i, w_j} = v_i$. Also, we set the global budget $b = W$. Then, for this $sMQ$ instance, we want to achieve an assignment $x$ of some pairs of subtask and worker that maximizes the task quality $\sum_{\forall <\tau_i, w_j> \in x } q(<\tau_i, w_j>)$ subjected to $\sum_{\forall <\tau_i, w_j> \in x }c_{\tau_i, w_j} \leq b$.
%
%    Given this mapping, we can show that the 0-1 knapsack problem instance can be solved, if and only if the transformed $sMQ$ problem can be solved.
%
%    This way, we can reduce 0-1 knapsack problem to the $sMQ$ problem. Since 0-1 knapsack problem is known to be NP-hard ~\cite{vazirani2013approximation}, $sMQ$ is also NP-hard, which completes our proof.
%\end{proof}

%\begin{definition}
%{\bf Maximum Coverage with Group Budgets (MCG {\it in short})}~\cite{DBLP:conf/approx/ChekuriK04}. Given a collection $S$ of a ground set X, $S = \left\{S_1, ..., S_p\right\}$, and a set of disjoint groups $G_1, ... , G_l$, of which each group $G_i$ is a subset of $S$.
%In addition, given an integer $k$, and an integer bound $k_g$ for each group $G_g$. A solution of MCG is a subset $H \subseteq S$ such that $|H| \leq k$ and $|H \cap G_g | \leq k_g$ for $1 \leq g \leq l$. The objective is to find a solution such that the number of elements of $X$ covered by the sets in $H$ is maximized.
%\end{definition}
%
%
%\begin{lemma}
%The $sQM$ problem is NP-hard.
%\end{lemma}
%
%\begin{proof}
%To prove $sQM$ is NP-hard, we show a polynomial reduction of the $MCG$ problem to our problem.
%
%Consider an instance of $MCG$ problem with a ground set $X = \left\{\tau_1, \tau_2, ..., \tau_m, w_1, w_2, ..., w_n \right\}$ and $S$ being a set of two-element subsets of $X$,i.e., $S = \left\{ \left\{ \tau_i, w_j \right\} : \tau_i \in X, w_j \in X \right\}$. Let $c$ be a cost function such that $c( \left\{ \tau_i, w_j\right\}) ( i = \left\{1, ..., m\right\}$  and  $j =  \left\{1, ..., n\right\})$. Group $G_i$ is a subset of $S$, i.e., $G_i = \left\{  \left\{ \tau_i, w_j\right\} : w_j \in X \right\}, i = \left\{ 1, 2, ..., m\right\}$.
%
%We reduce such instance of $MCG$ problem to the $sMQ$ problem as follows. In our problem, we divide the task completion time $\tau_t$ into $m$ time slots, then task of each time slot can be treated as a subtask. Let $\tau = \left\{ \tau_i : i = 1, ..., m\right\}$ be the set of these subtasks, and $W =\left\{w_j : j = 1, ..., n \right\}$ be the set of workers and we are also given an cost constraint $Budget$. Each element of $S$ denotes the corresponding $\tau_i$ is assigned to $w_j$. The cost that task $\tau_i$ is executed by worker $w_j$ is equal to $c_{\tau_i, w_j} = c( \left\{ \tau_i, w_j\right\})$. For a subtask $\tau_i$, it can be executed by anyone of the workers $W$, so we define each group $G_i$ denotes the pairs of task $\tau_i$ and all the worker $W$, $G_i = \left\{  \left\{ \tau_i, w_j\right\} : w_j \in W \right\},\ i = \left\{ 1, 2, ..., m\right\}$. Consequently, to solve $sMQ$ problem, we need to find a subset $I$ of maximum cost $Budget$ whose $Quality$ is maximized. Clearly, if an answer to $sMQ$ is the set $I$, the answer to $MCG$ will be the set of $H \subset S$ of maximum $Quality$ such that $c(H) \leq Budget $ and $ | H \cap G_i| \leq k_i = 1$ for $1 \leq i \leq m$, here $c(H)$ denotes the total cost of each element of $H$ and $k_i = 1$ denotes a subtask can only be completed by a worker. Hence, the $MCG$ problem can be reduced to our problem and so our problem is NP-hard.
%\end{proof}

%------------------------------------------------
\subsection{Approximation Algorithms}
\label{sec:single_alg}

\newcommand{\Tau}{\mathrm{\it T}}

%It is not possible to find a polynomial time solution for the optimal assignment, since the $sMQ$ problem is NP-hard.
Hereby, we provide a suboptimal solution with guaranteed approximation ratios, based on the submodular property of the quality metric, as discussed in Section~\ref{subsec:property}.
Since the problem is of budgeted maximization for a submodular function, we can have a heuristic algorithm, which repeatedly selects an element (e.g. a subtask) that maximizes the quality increment until the budget is exceeded. The process is detailed in Algorithm~\ref{alg:single}.

%%%%%%%%%%%%%%% commented by XXK on Jan 23 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{algorithm}
%\label{alg:single}
%\caption{Single task assignment algorithm} %of single task assignment
%%\begin{algorithmic}[1]
%\LinesNumbered
%\KwData{$b>0$, a set of workers $W$, a task $\tau$}
%%\KwOutput{a task assignment matrix $x$;}
%%\Ensure a task assignment matrix $x$;
%%\State prune workers over the limited $Budget$ by Lemma \ref{prune2};
%% \State divide the task $\tau$ into $m$ subtasks, $\tau_i \in \tau$, $1\leq i \leq m$
%%\State initialize $f(\tau_i) = 0$, for all $\tau_i \in \tau$
%%\State get the set of online workers $W_i$ for each subtask $\tau_i$ by Lemma \ref{prune1};
%%\For{each subtask $\tau^{(j)}$}
%%{
%%    Find the nearest worker and compute the corresponding cost $c(\tau^{(j)})$\;
%%}
%Initialize the states of subtasks $\{\tau^{(j)} \in \tau \}$ as {\tt NULL} \;
%For each subtask $\tau^{(j)}$ get the corresponding cost     $c(\tau^{(j)})$\;
%Execute the subtask $\tau^{(h)}$ yielding the highest quality but not exceeding the budget, $T_{cur} \leftarrow T_{cur} \cup \tau^{h}$\;
%%Select the subtask $\tau^{(r)}$ yielding the highest proportion of quality to cost and set its state from NULL to Executed\;
%%Initialize $x^2_{\tau^{(j)},w}=0$ for all $\tau^{(j)} \in \tau $, $w \in W_i$\;
%\While{$C(\tau) \leq b$}%$\tau \neq \emptyset $ and
%{
%    \For{ $ \tau^{(j)} \in \tau - T_{cur}$ }
%    {
%            Compute $\frac{q(\Tau_{cur} \cup  \tau^{(j)}) - q(\Tau_{cur})}{c(\tau^{(j)})}$\;
%            %$ \frac{\Delta q(\taux_{\tau^{(j)}})}{C(x_{\tau^{(j)}}) } $\;
%    }
%    $\tau^{(*)} \leftarrow argmax\left\{ \frac{\Delta q(\tau)}{c(\tau^{(*)}) } : \tau^{(*)} \in \tau \right\}$\;
%    %$x^2_{\tau^{(r)}, w^{(r)}} \leftarrow 1$;
%    Update $\tau^{(*)}$'s state to {\tt Executed}\;
%    $T_{cur} \leftarrow T_{cur} \cup \tau^{(*)}$\;
%    %$\tau \leftarrow \tau \backslash \tau^{(*)}$\;
%}
%return $T_{cur}$ as the final result\;
%%$x$ with the highest task quality, $x \in \left\{x^1,x^2\right\} $\;
%\end{algorithm}

\begin{algorithm}
\label{alg:single}
\caption{Single task assignment algorithm} %of single task assignment
%\begin{algorithmic}[1]
\LinesNumbered
\KwData{$b>0$, a set of workers $W$, a task $\tau$}
Initialize the states of subtasks $\{\tau^{(j)} \in \tau \}$ as {\tt NULL}  and initialize $T_{cur}'$ and $T_{cur}$ as two empty sets\;
For each subtask $\tau^{(j)}$ get the corresponding cost     $c(\tau^{(j)})$\;
Execute the subtask $\tau^{(h)}$ yielding the highest quality but not exceeding the budget, $T_{cur}' \leftarrow \{ \tau^{(h)} \}$\;
\While{$C(\tau) \leq b$}%$\tau \neq \emptyset $ and
%\While{$ q(\tau) \leq Q$}
{
    \For{ $ \tau^{(j)} \in \tau - T_{cur}$ }
    {
            Compute $\frac{q(\Tau_{cur} \cup  \tau^{(j)}) - q(\Tau_{cur} )}{c(\tau^{(j)})}$\;
            %$ \frac{\Delta q(\taux_{\tau^{(j)}})}{C(x_{\tau^{(j)}}) } $\;
    }
    $\tau^{(*)} \leftarrow argmax\left\{ \frac{\Delta q(\tau)}{c(\tau^{(*)}) } : \tau^{(*)} \in \tau \right\}$\;
    Update $\tau^{(*)}$'s state to {\tt Executed}\;
    $T_{cur} \leftarrow T_{cur} \cup \tau^{(*)}$\;
}
return $T_{cur}'$ or $T_{cur}$ with the highest quality as the final result\;
\end{algorithm}

Hence, the heuristic value is defined as the quality increment divided by the corresponding cost.
Let the currently assigned set of subtasks be $\Tau_{cur}$.
At each iteration, the algorithm greedily selects a subtask $\tau^{(*)}$ from the set $\tau - \Tau_{cur}$, such that the heuristic value is maximized.
Formally, the greedy rule is to find a subtask $\tau^{(*)}$ as follows.
\begin{align}
\small
\tau^{(*)} & = \underset{\tau^{(j)}}{argmax } \frac{\Delta q(\tau)}{c(\tau^{(j)}) } = \underset{\tau^{(j)}}{argmax} \frac{q(\Tau_{cur} \cup  \tau^{(j)}) - q(\Tau_{cur})}{c(\tau^{(j)})} \nonumber
\end{align}
%%%%%%%%%%%%%%% xk commented at June 9 %%%%%%%%55%
%\begin{align}
%\small
%\tau^{(*)} & = argmax_x \frac{\Delta q(\tau)}{C(\tau) } = argmax_{i,j} \frac{q(\Tau_{cur} \cup  \tau^{(j)}) - q(\Tau_{cur})}{C(\tau^{(j)}, w_i^{(j)})} \nonumber
%\end{align}

%worker-and-subtask assignment, $x_{\tau^{(j)}, w_i^{(j)}}$, which maximizes the quality increment, $\Delta q$, together with the lowest cost.
%Formally, the greedy rule is to find an assignment $x^*$ as follows.
%\begin{align}
%\small
%x^* & = argmax_x \frac{\Delta q(x)}{C(x) } = argmax_{i,j} \frac{q(\Tau_{cur} \cup  \tau^{(j)}) - q(\Tau_{cur})}{C(\tau^{(j)}, w_i^{(j)})} \nonumber
%\end{align}

\begin{figure*}
  \centering
  \includegraphics[height=2.2in,width = 2.1\columnwidth]{fig/fig2.pdf}

  \caption{An Example. ($k=2$, $t_s = 4$, $m=100$): (a) Current state $T_{cur}$; (b) $2$-Nearest Neighbors; (c) $1$-dimensional Order-$2$ Voronoi Diagram; (d) Tree-structured Index; (e) Auxiliary Information.}

  \label{fig:voronoi}
\end{figure*}

We use an example to illustrate the process.
%Assume a TCSC task consisting of a set of subtasks.
Assume that there are $4$ executed subtasks, i.e., $T_{cur} = \{ \tau^{(2)}, \tau^{(4)}, \tau^{(7)}, \tau^{(9)} \}$, of a TCSC task, represented by shaded slots, as shown in Fig.~\ref{fig:voronoi} (a).
%Given the set of currently executed subtasks $T_{cur} = \{ \tau^{(2)}, \tau^{(4)}, \tau^{(7)}, \tau^{(9)} \}$ (Fig.~\ref{fig:voronoi} (a)),
Algorithm~\ref{alg:single} enumerates all remaining slots/subtasks.
At each iteration, a slot is selected for tentative execution in order to find the one with the highest heuristic value.
If $\tau^{(1)}$ is chosen and tentatively executed, $\rho(\tau^{(1)})$ is reduced to $0$ and the heuristic value increment is $0.0016$.
However, if $\tau^{(5)}$ is tentatively executed, $\tau^{(6)}$'s $2$-NN result is changed from $\{\tau^{(4)}, \tau^{(7)}\}$ to $\{\tau^{(5)}, \tau^{(7)}\}$.
Therefore, both $\rho(\tau^{(5)})$ and $\rho(\tau^{(6)})$ should be recalculated for getting the quality and the heuristic values.
The process is repeated for all the unexecuted slots. Finally, $\tau^{(1)}$ is selected, since it derives the maximum heuristic value in this example.

By setting the greedy strategy as such, Algorithm~\ref{alg:single} guarantees a $(1-1/\sqrt{e})$ approximation to the optimal solution, as shown in \cite{article}.
%In our problem, the function refers to the proposed quality metric and the process refers to the dynamic allocation of subtasks.
%The process is detailed in Algorithm~\ref{single-alg1}.

%%%%%%%%%%%%%%%%% Xike xommented in June 15 %%%%
%The correctness is proved by Lemma~\ref{lem:approx}.
%
%\begin{lemma}
%\label{lem:approx}
%Algorithm~\ref{alg:single} achieves a $(1-1/\sqrt{e})$ approximation ratio to the optimal solution.
%\end{lemma}

%\begin{proof}
%To be updated.
%{\bf we emphasize the difference of set cover problem, then refer to \cite{khuller1999budgeted} for proving the correctness.}
%
%Here, we use $\Tau_i$ to denote task assignments at each iteration $i$ to Algorithm~\ref{alg:singlej}, and $OPT'$ contains the task assignment of $OPT$ and $\Tau_i$. Using the monotonicity of $q(\tau)$, we have $q(OPT)- q(\Tau_i) \leq q(OPT') -q(\Tau_i)$. For each time slot $e \in {OPT-\tau_i}$, it has $ Z_j = q(\Tau_i \cup e) - q(\Tau_i)$. Then $q(OPT)- q(\Tau_i) \leq \sum Z_j$.
%\end{proof}

%{\bfseries The task finishing quality ratio}: Before we present the greedy algorithm, we first define the increase per unit-cost, $ Quality(\tau_i)^*$, of task finishing quality $Quality(\tau)$, in the case where we assign a worker $w_j$ to the unexecuted subtask $\tau_i$. Specifically, we define the task finishing quality ratio after assigning worker $w_j$ to unexecuted sub-task $\tau_i$ as follows:
%
%\begin{equation}\label{7}
%\begin{aligned}
%  &q = \frac{Quality(\tau_{new}) - Quality(\tau_{old})}{TC(x_{\tau_i})} \\
%\end{aligned}
%\end{equation}
%Where subtask $\tau_i$ is executed in task $\tau_{new}$, $f(\tau_i) =1$, $ \tau_i \in \tau_{new}$, while subtask $\tau_i$ is unexecuted in task $\tau_{old}$, $f(\tau_i) =0$, $\tau_i \in \tau_{old}$.

%        {\bfseries Approximation algorithm}:
%        According to the definition of the task finishing quality ratio $Quality(\tau_i)^*$, we propose a approximation algorithm, which iteratively assigns a worker to a subtask that can always achieve the highest task finishing quality ratio.




%Each worker has a trajectory which is uploaded before, then there may exists some workers who far away from the task that the traveling cost to perform the task for these workers is beyond the limited $Budget$. Thus, we first prune high-cost workers in Line 1. Next, considering the features of spatiotemporal continuous task, we divide the task into $m$ subtasks so that each subtask can be executed by one worker in Line 2. And initialize all subtasks are unexecuted in Line 3. According to the Definition \ref{worker}, the subtask can only be performed by those workers who are in online mode, and the mode of workers will change over time. Thus, we select online workers $W_i$ that can be assigned to subtask $\tau_i$ in Line 4.

%{\bf to-be-deleted}Our algorithm is to select the highest task finishing quality ratio when performing subtask $\tau_i$. From the Formula \ref{7}, the lower the traveling cost that worker is assigned to subtask $\tau_i$, the higher the task finishing quality ratio. Obviously, this process is to find the worker $w_{(i)}$ nearest to subtask $\tau_i$ at time slot $i$(considering the cost function in Definition \ref{cost}). Here, we create index to do this work in Line 5. In Line 6-7, Algorithm 1 select the best subtask solution as alternative to the output, which have been proved to guarantees a constant factor approximation\cite{khuller1999budgeted}. In Line 9-20, selecting the subtask $\tau_x$ whose task finishing quality ratio is maximum for each iteration until the total traveling cost reaches the limited $Budget$. In Line 21, Algorithm 1 returns task assignment matrix $x$ whose task finishing quality is maximized as task assignment result and $x \in \left\{x^1,x^2\right\}$.
%
% {\bfseries Pruning strategies}: The task finishing quality ratio can be used as a measure to evaluate and decide which worker-and-subtask assignment pair should be added to the task assignment. That is, each iteration our greedy algorithm aims to choose one worker-and-subtask assignment pair with the highest task finishing quality ratio. However, it is not efficient to enumerate all valid worker-and-subtask assignment pairs and compute task finishing quality ratio. In the worst case, the time complexity is as high as $O(m �� n)$, where $m$ is the number of subtasks and $n$ is the number of workers. Therefore, we first prune the workers and some time slots of task according to the fixed $Budget$.
%
%
%        \begin{lemma}
%        \label{prune1}
%        (Pruning Offline Workers) Given a set of workers $W$, a worker can perform task only when he is online. Here, we define $W_i$ be the set of online workers at time slot of subtask $\tau_i$, then we can safely prune those offline workers.
%        \end{lemma}
%
%        \begin{lemma}
%        \label{prune2}
%        (Pruning High-Cost Workers) Each worker $w_j$ has a known trajectory, $w_j \in W$, and we can get the minimum distance between worker $w_j$ and task $\tau$. From Definition \ref{cost}, it is easier to compute the minimum traveling cost. If the minimum traveling cost is greater than the limited $Budget$, then we will not assign worker $w_j$ to task $\tau$.
%        \end{lemma}
%
%        \begin{lemma}
%        \label{prune3}
%        (Pruning Subtasks with Insufficient Budgets) Let $\widetilde{c}$ be the total traveling cost for those worker-and-subtask assignment pairs. If the minimum traveling cost $TC(\tau_i)_{min}$ for the unexecuted subtask $\tau_i$ is greater than the remaining budget ($Budget-\widetilde{c}$), then we can safely prune subtask $\tau_i$.
%        \end{lemma}
%
%        \begin{lemma}
%        \label{prune4}
%        (Pruning Subtasks which is impossible to be performed) let $\tau_a$, $\tau_b$ be the unexecuted subtasks, and if there exists  $Quality(\tau_a)^* > Quality(\tau_b)^*$, $TC(\tau_a)<TC(\tau_b)$. According to the traveling cost of each subtask, we can get the range of the number of executed subtasks. Let $h$ be the maximum number of executed subtasks. Thus, if the number of subtask $\tau_a$ satisfying these two conditions is higher than $h-\tau_e$ at a iteration, the subtask $\tau_b$ can be pruned.
%        \end{lemma}
%
%        To summarize, by utilizing Lemmas \ref{prune1}, \ref{prune2}, \ref{prune3} and \ref{prune4}, we can effectively filter out those workers and subtasks that do not meet the limited $Budget$, which can significantly reduce the number of times to compute the task finishing quality ratio.
%
%
%%    {\bfseries Selecting the nearest free worker}: In order to maximum the task finishing quality ratio, we need to select the free worker whose travel cost is minimum, more simply, that is to select the free worker nearest to the subtask for each iteration. As the number of workers may be huge, we create R-tree \cite{papadopoulos1997performance} based on the location of workers and task for each time slot.
%
%Next, we present the time complexity of the approximation algorithm.

{\bfseries Complexity Analysis}. First, the number of iterations, i.e., the outer loop of Algorithm~\ref{alg:single} (line $4$), is at the level of $O(m)$. Second, the inner loop (line $5$) is at the level of $O(m)$, since one needs to try all $m$ subtasks and get their heuristic values in order to find the one maximizing the overall quality.
Third, for each trial of a subtask, one needs to calculate the corresponding heuristic value, i.e., the overall quality increase of implementing the subtask, according to the quality metric function. The overall quality increase is the summation of individual quality increments of all other $m-1$ subtasks, so the complexity is $O(m)$ (line 6).
Fourth, for quality increment of a individual subtask, $k$ timeslots in the neighborhood should be visited.
In our implementation, we maintain a sorted list for subtasks that are sorted in the ascending order of the corresponding time slots.
During the query evaluation, $O(log(m))$ cost is used for finding the nearest assigned subtask, and then $O(k)$ cost is used for refining the exact $k$-NN.
%More, if workers are spatially indexed, the time cost of finding a nearest worker for a subtask is expected to be $O(log(n))$, where $n$ is the total number of workers.
Therefore, the total time complexity is $O(m^3log(m))$.

In summary, the approximation algorithm gives a polynomial alternative for tackling the NP-hard optimization problem. However, the computational overhead makes it impractical in real-time task assignment scenarios. In the sequel, we propose a series of techniques for better efficiency and scalability.

\subsection{Efficient Heuristic Value Calculation}
\label{subsec:eff}

%\begin{figure}
%\centering
%\subfigure[Finishing subtask $\tau^{(3)}$] {\includegraphics[height=0.8in,width=1.6in]{fig/error(1).pdf}}
%\subfigure[Finishing subtasks $\tau^{(3)}, \tau^{(6)}$] {\includegraphics[height=0.8in,width=1.6in]{fig/error(2).pdf}}
%\caption{The computation of $k$-NN error(assume $k=2$)}
%\label{fig:error_compute}
%\end{figure}

%\begin{figure*}
%\centering
%\subfigure[The $k$-NN neighbour for each subtask]{
%    \begin{minipage}{9cm}
%    \includegraphics[height=1.5cm,width=6.5cm]{fig/tree(1).pdf}
%   % \caption{The $k$-NN neighbour for each subtask}
%    \end{minipage}
%}
%
%\subfigure[Node information]{
%    \begin{minipage}{8cm}
%    \includegraphics[height=2.5cm,width=7cm]{fig/tree(3).pdf}
%    %\caption{Node information}
%    \end{minipage}
%}
%\subfigure[Tree structure]{\includegraphics[height=4.5cm,width=8.5cm]{fig/tree(2).pdf}}
%\caption{Tree-based heuristic value calculation(assume $ts = 4, k = 2$)}
%\end{figure*}

%For example, we calculate the error of subtask $\tau^{(4)}$ when the execution is shown as Fig \ref{fig:error_compute}, respectively. In Fig \ref{fig:error_compute}(a), the number of executed subtask less than $k$, then $\rho_{err}(\tau^{(4)}) = \frac{1}{2} + \frac{|\tau^{(3)},\tau^{(4)}|_i}{2m} = \frac{7}{12}$. After executing a new subtask $\tau^{(6)}$(Fig \ref{fig:error_compute}(b)), the number of executed subtask equals $k$, and $\rho_{err}(\tau^{(4)}) = \frac{|\tau^{(3)},\tau^{(4)}|_i + |\tau^{(4)},\tau^{(6)}|_i}{2m} = \frac{1}{4}$.



The idea of accelerating the algorithm is in two parts.
First, for finding the maximum heuristic value, how to avoid unnecessary enumeration of all $m$ subtasks.
Second, the calculation of a heuristic value refers to the summation of partial qualities of all subtasks. For the heuristic value calculation, how to maximally reuse the computation so as to avoid unnecessary checking of all time slots.
%Second, how the effect of quality increment, so that the recalculation of the quality value, as well as the heuristic value, can be reduced to a subinterval, instead of all the $m$ slots?

%\begin{figure}
%\centering
%\includegraphics[height=2.5cm, width=5cm]{fig/knn.pdf}
%\caption{The locality of $k$-NN searching}
%\label{knn_locality}
%\end{figure}

{\bf Locality of $k$-NN Searching.} We try to scale down the problem by considering the locality of $k$-NN searching. We observed from Fig.~\ref{fig:voronoi} (b) that if two slots are proximate, their $k$-NN results tend to be similar. For example, $\tau^{(1)}$ and $\tau^{(2)}$ share the same $k$-NN results, i.e., $\{\tau^{(2)}, \tau^{(4)}\}$.
%In the example of Fig.\ref{knn_locality}, all time slots are divided into three sets, denoted as ${s_1,s_2,s_3}$. The $k$-NN results of time slot within a set is the same. As the inserting time slot belongs to the set $s_2$, it would not change the heuristic value of time slots which belong to other set except $s_2$. {\bf fig should be updated}
Theoretically, the solution space of $k$-NN searching over the $m$ subtasks is a one-dimensional order-$k$ Voronoi diagram. The domain space is a one-dimensional interval, i.e., from $1$ to $m$. The diagram splits $m$ slots into disjoint intervals, called Voronoi cells, such that the $k$-NN searching provides the same result if queries are within the same Voronoi cell. In Fig.~\ref{fig:voronoi} (c), for example, the Voronoi cell $V(\tau^{(2)}, \tau^{(4)})$ covers slots from $\tau^{(1)}$ to $\tau^{(4)}$, meaning that all slots from $\tau^{(1)}$ to $\tau^{(4)}$ take $\{\tau^{(2)}, \tau^{(4)}\}$ as their $2$-NN results.

Such a structure facilitates the algorithm evaluation in two aspects. First, the time cost for $k$-NN searching can be reduced from $O(log(m))$ to constant time $O(1)$, as the diagram pre-computes the solution space for the $k$-NN queries. Second, the diagram accelerates the calculation of heuristic values.
For the tentative execution of a subtask, the heuristic value is calculated by enumerating all other slots which takes $O(m)$ (Algorithm~\ref{alg:single}, line 6).
%Originally, it takes $O(m)$ by enumerating all other $m-1$ slots to get the heuristic value for one slot (Algorithm~\ref{alg:single}, line 6).

Recall that the finishing probability of an unexecuted subtask depends on its $k$-NN interpolation. So, the value of finishing probability of an unexecuted subtask does not change, if the order-$k$ Voronoi cell to which it belongs does change, with the tentative execution.
%It shows that the partial quality of a slot does not violate, as long as its belonging Voronoi cell does not change with the tentative slot execution.
This way, the problem of quality increment calculation is transformed to the reformulation of Voronoi cells w.r.t. the tentative subtask execution, which can be handled locally, since the diagram handles such updates locally~\cite{voronoi-book}. We cover more details below.

The technical challenge arising is that there could be a large number of order-$k$ Voronoi cells, making the gains of local computation not worthy of the overhead of the Voronoi diagram construction.
In particular, the average number of order-$k$ cells is $O(k(m-k))$~\cite{voronoi-book}.

{\bf Approximated One-dimensional Voronoi Diagram.} To handle that, we propose an approximate version of one-dimensional order-$k$ Voronoi diagram. The idea is to use an aggregated binary tree for Voronoi cell indexing and Voronoi diagram approximation (Fig.~\ref{fig:voronoi} (d)).
In the tree, each node represents a time segment $[l, r]$, where $l$ and $r$ are for the two slots on the segment's left and right ends, respectively. The root node is the interval of the entire $m$ slots. For each node, we store the auxiliary information in the form of a quadruples, i.e., $\langle k$-$set, knn(l), knn(r), q' \rangle$, as shown in Fig.~\ref{fig:voronoi} (e).

The $k$-set of a node is the union of $k$-NN results for all its offsprings.
%The elements in $k$-set are sorted.
%In particular, we use $[l_{ks}, r_{ks}]$ to represent the range, where $l_{ks}$ ($r_{ks}$) is the lowest (highest) value of the corresponding time segment.
$knn(l)$ and $knn(r)$ are $k$-NN results of the two end slots. The $k$-NN results are sorted in ascending order of the distance to $l$ (or $r$), so that the distance from $l$ (or $r$) to its $k$-th nearest neighbor can be fast retrieved, denoted by $k_{max}(l)$ (or $k_{max}(r)$). So, we can derive the influence range of a node as $[max(1, l-k_{max}(l)), min(m, r+k_{max}(r))]$, such that the quadruple of the node can be affected if a tentatively executed slot is within the influence range.
$q'$ is the partial quality value of the node.
For subtask $\tau^{(j)}$, its partial quality equals $p^{(j)}log(p^{(j)})$.
The quality of a node is the summation of partial qualities of all subtasks in its offspring.
%The overall tree structure is like an aggregated binary tree.
This way, the quality value can be fast retrieved by querying the upper level nodes of the tree structure. Upon updating, only necessary subtrees are retrieved and revised, following the style of updating an aggregated tree-structure.

%{\bf How the tree is used for solving the k-NN problem in quality calculation?}
{\bf Maximum Heuristic Value Calculation.}
With the tree structure, it takes much less computational overhead than enumerating all $m$ slots. The process is implemented by traversing the tree in a best-first manner with an associated heap. The elements of the heap are tree nodes which are sorted in descending order of the upper bounds. The higher an element ranks in the heap, the more likely it corresponds to the maximum heuristic value increment.

Next, we study how to upper bound the effect of a tentative insertion.
A tentative insertion affects the $k$-NN interpolation results so the quality value varies. The effect can be categorized into {\it inter-node} and {\it intra-node} cases\footnote{We consider the leaf node for ease of presentation. The calculation of upper bounds for non-leaf nodes can be done in a bottom-up manner, as the construction process of an aggregated tree-structure.}.

For the intra-node case, if an unexecuted slot is tentatively executed, of the same node, another unexecuted slot's $k$-th NN distance is reduced to $1$ at most. It corresponds to the extreme case that the slot is next to the tentative executed slot, whereas the distance between them is $1$. So, the interpolation error ratio can be lower bounded as follows.

%\begin{lemma}
%({\bf Lower Bound for Interpolation Error Ratio.})
\begin{align}
\small
\label{eqn:lb}
\rho_{err}(\tau^{(j)}) \geq \frac{1}{k\cdot m} [\sum_{e \in S_{(k-1)NN}(\tau^{(j)})} |e, \tau^{(j)}|_i + 1]
\end{align}
%\end{lemma}

%The proof is omitted due to page limits.
%\begin{proof}
%If an executed slot is executed, the $k$-th NN distance of unexecuted slots of the same node can be reduced to $1$ at most. Therefore, the interpolation error of unexecuted slots is equal to $k-1$ NN distance plus $1$.
%\end{proof}

Therefore, the upper bound of a node's quality can be derived by the lower bound of $\rho_{err}$ (Equation~\ref{eqn:lb}), since the value of $q(.)$ is inversely proportional to that of $\rho_{err}(.)$. So, the upper bound of a node's heuristic value is calculated by the maximum quality change divided by the minimum cost of all unexecuted subtasks in the node.

For the inter-node case, a tentatively executed slot of a node would also change the $k$-NN interpolation result of other nodes. For example, in Fig.~\ref{fig:voronoi} (d), we have two leaf nodes, $n_1$ and $n_2$. If $\tau^{(3)}\in n_1$ is tentatively executed, $\tau^{(5)}\in n_2$'s second nearest neighbor changes from $\tau^{(7)}$ to $\tau^{(3)}$. The corresponding quality value change should also be incorporated and updated.

%%%%%% xk commented 0606 %%%%%%%%%%%%
%The calculation of the upper bound is shown in Lemma~\ref{lem:ubh}.

%\begin{lemma}
%\label{lem:ubh}
%({\bf Upper bound of Heuristic Values.})
%For unassigned slots, $k$-th NN distance minus $1$, the slot with minimum $p$ is selected and replaced with $\frac{1}{m}$. The minimum cost of the node is selected.
%\end{lemma}
%
%Finishing a new subtask will change the quality of other subtask. We obtain the upper bound of node $n_1$ by calculating the quality variation of node $n_1$ and other nodes. We assume the $k$NN interpolation distances of each subtask $\tau_i$ in node $n_1$ is $I_{\tau_i}$, and $k$-NN interpolation distances is $I_{\tau_i}^k$ .
%
%From Equation 3 and 4, we get the quality variation is caused by the change of $k$-NN interpolation distances. First, we try to calculate the quality variation of node $n_1$, and it is also calculating the change of $k$-NN interpolation distances. When selecting a subtask to be executed, one of these unexecuted subtask will be selected, and its interpolation distances become 0; while the $k_{th}$ NN interpolation distance of other subtasks reduces to 1, its interpolation distances are $I_{\tau_i}- I_{\tau_i}^k + 1$, as the new executed subtask is closest to other subtasks.
%
%Meanwhile, Finishing a subtask in node $n_1$ will also change the $k$-NN neighbours of other nodes, and the $k_{th}$ NN interpolation distance of node $n_o$ becomes $min(I_{\tau_i}, |n_1, n_o|_t)$, $|n_1, n_o|_t$ denotes the time interval between nodes $n_1$ and $n_o$.
%
%Based on the above description, we have calculated the maximum quality variation of node $n_1$, then we attempt to find the minimum cost in node $n_1$. At last, we could get the upper-bound of node $n_1$.


At each iteration, the top element of the heap is popped up and the child nodes are inserted. If the top element is a time slot/subtask, the exact heuristic value increase can be obtained. Suppose the value is $\theta$.
Then, all other elements in the heap whose upper bounds are below $\theta$ can be pruned. The process repeats until the heap is empty. The slot that gives the maximum heuristic value is then obtained.

The advantages of using the tree structure are two-fold. First, using best-first searching for obtaining the slot with the potentially maximum heuristic value is expected to take $O(log(m))$ time.
Second, the locality of $k$-NN searching is reflected by the decomposition of tree leaf nodes.
Suppose that calculating the updated heuristic value of a leaf node takes constant time.
Then, instead of enumerating $O(m)$ slots for calculating the updated heuristic value, one takes $O(log(m))$ time to retrieve and update the relevant leaf nodes, reducing the corresponding computation overhead from $O(m)$ to $O(log(m))$.
The overall cost is $O(mlog^3(m))$.
%Next, we discuss how the tree structure is constructed.

%Solution: we have to go through the m elements to decide which one gives best $\Delta$ quality / cost;
%For a node, if its k-set's value range has no overlap with an element, no need to recalculate the node plogp table.
%Otherwise, find all nodes whose k-set's value range covers e', and calculate the summation of $\Delta$ quality
%Then, for an element e', since we know its cost and its corresponding quality change, we can do pruning to test fewer elements

{\bf Tree Construction.}
We consider the tree construction in an incremental manner.
Suppose that a time slot $e$ is to be tentatively executed, meaning that $e$ is with the maximum current heuristic value.
The process of tree construction is triggered accordingly, and is revoked recursively.
At each iteration, we test if a subtree will be affected. If yes, we update the associated quadruples and forward the updates to the descendants. Otherwise, the entire subtree is skipped.

%When the number of assigned slots is greater than $k$,
We summarize two cases to determine whether the current node will be affected and therefore updated by the tentative execution. Based on that, we can disqualify irrelevant nodes at a higher level to save the overhead of the tree construction.
%A subtree can be pruned for the structure adjustment, if it is detected to be not affected by the insertion. As will be shown, such pruning techniques save not only the overhead of tree construction, but also the quality increment calculation.
%Notice that the elements should always be incorporated if the set of currently assigned time slots is less than $k$.

%There can several cases that the element $e$ should be considered for the current time segment $[l, r]$.

\begin{itemize}
\item \emph{Case 1.} A node will be affected, if the tentatively executed slot is within the influence range of the node.
%\item \emph{Case 2.} A node will be affected, if its corresponding $kNN(l)$ or $kNN(r)$ changes by incorporating $e$.
\item \emph{Case 2.} A node will not be affected, if its parent node is not affected, by $e$.
\end{itemize}

%Cases $1$ and $3$ are intuitive and corresponding discussion is omitted due to page limits. %For Case $2$, we have to prove two things to show its correctness {\bf refer to the lemma}.

By doing so, we can find appropriate nodes for updating.
%For the efficient determination of Case 2, we use $k$NN distance, i.e., the distance to $k$-th nearest neighbor (for a segment's end point). Given the new slot $e$, we can simply test if the slot is within the current $k$NN distance.
The updates can thus be propagated to the leaf level so that the node splitting should be handled.

{\bf Splitting and Stopping Conditions.}
During splitting, a node is decomposed into two sub-nodes, with its time segment split into two equal sized sub-segments.
The quadruple of the node can thus be partially inherited by its sub-nodes.
For example, the left sub-node inherits the $knn(l)$ of its parent, because they share the same left end slot.
In particular, we consider two stopping conditions.
\begin{itemize}
\item \emph{Condition 1.} For a node with segment $[l, r]$, splitting stops, if $knn(l) = knn(r)$.
\item \emph{Condition 2.} If the length of a node's segment is smaller than a pre-specified threshold, $t_s$, splitting stops.
\end{itemize}
Condition $1$ guarantees that current segment belongs to the same order-$k$ Voronoi cell, so that there is no need for further splitting. Condition $2$ limits the depth of the tree structure to $\lceil log_{t_s}(m) \rceil$. It serves as a knob for tuning the approximation accuracies so as to control the construction overhead of the tree structure.
The correctness of Conditions $1$ is guaranteed by Lemma~\ref{lem:cond1} (in Appendix~\ref{subsec:cond1}).
%Cases $1$ and $3$ are intuitive, so that the discussion is omitted due to page limits.

%\begin{proof}
%We prove that by contradiction.
%Suppose a slot $e'$ on the segment, $e' \in [l, r]$, such that $kNN(e') \neq kNN(l)$. It means that there exist a slot $a$,
%
%Suppose a slot $e'$ such that $kNN(e')\neq kNN(l)$, $ e' \in [l, r]$. $|e', r| \leq |l,r|$, the time slots of $kNN(e')$ is closer to $r$ compared to  $kNN(l)$. Then, $ kNN(r) = kNN(e')$, and $ kNN(l) \neq kNN(r)$, thus the lemma is true.
%\end{proof}

%\begin{lemma}
%For a new slot $e$, $e \notin [l, r]$, and $kNN(l)$ or $kNN(r)$ would change if incorporating $e$, the segment will be affected by $e$.
%\label{lem:case2}
%\end{lemma}
%
%\begin{proof}
%Clearly, the new slot $e$ will change $kNN(l)$ or $kNN(r)$, and Condition 1 does not satisfy, so the time segment will split.
%\end{proof}

%%%%%%%%%%%%%%%%%%%% commented by Xike %%%%%%%%%%%%%%%%%%%%%%%%
%{\bf Pruning.}
%Given a new element $e$ to be inserted and a time segment, if none of the slots on the segment takes $e$ as its $k$-NN. The segment will not be affected by $e$.
%
%Property:
%For a node¡¯s k-set with value range $[l_ks, r_ks]$, if the new element e¡¯ is beyond the range, it means the quality table of node takes no change with the arrival of e¡¯.
%So, we scale down the problem from calculating plogp for all m slots, into those unpruned nodes. The process is similar to a range query, and thus takes complexity of O(log m).
%
%In implementation, we mark the $k$NN distance, i.e., the distance to $k$-th nearest neighbor, for each segment's end points. While determining the relationship between the segment and the new slot, we simply test if the slot is within the current $k$NN distance, so that the overhead of $k$NN evaluation can be saved for each comparison.
%
%For a node, represented by [l, r], if $kNN(l) \neq kNN(r)$, it splits;
%So, no splitting for the first k element insertion. (btw: 1/mlog(1/m)) can be precalculated.
%
%For a node¡¯s k-set with value range $[l_ks, r_ks]$,
%if the new element e¡¯ is beyond the range, it means e¡¯ can not be k-NN for any slot in [l, r], do nothing;
%Otherwise, store e¡¯ in the node¡¯s k-set, update k-NN(l) and k-NN(r) and repeat this for its decedents. If current node is a leaf-node, update its plogp table
%Notice that while traversing down, left node¡¯s left-end inherits its parent¡¯s left-end; right node¡¯s right-end inherits its parent¡¯s right-end.


%\subsection{An Improved Approximation Guarantee}
%     To achieve the same performance guarantee of $(1-1/e)$ which can be achieved for the unit-cost in the case of general submodular functions\cite{nemhauser1978analysis},we apply the algorithm in Khuller et.al.\cite{khuller1999budgeted} to our problem. The approximation algorithm first adopts a partial enumeration heuristic which enumerates all sets of up to $q$ subtasks for some constant $q>0$, and complements these subtasks by greedily adding the subtask whose task finishing quality ratio is maximum for each iteration until reaching the fixed $Budget$. They prove that this algorithm guarantees a $(1-1/e)$ approximation.
%
%    {\bfseries Approximation algorithm}: We show an improved algorithm as Algorithm \ref{single-alg2}.
%        \begin{algorithm}
%        \label{single-alg2}
%       Approximation algorithm 2 of single task assignment
%        \begin{algorithmic}[1]
%            \Require
%             $q>0$, $Budget>0$, a set of workers $W$, a spatiotemporal continuous task $\tau$;
%            \Ensure a task assignment matrix $x$;
%            \State prune workers over the limited $Budget$ by Lemma \ref{prune2};
%            \State divide the task $\tau$ into $m$ subtasks, $\tau_i \in \tau$, $1\leq i \leq m$
%            \State initialize $f(\tau_i) = 0$, for all $\tau_i \in \tau$
%            \State get the set of online workers $W_i$ for each subtask $\tau_i$ by Lemma \ref{prune1};
%            \State compute the minimum traveling cost $TC(\tau_i)_{min}$ for each subtask $\tau_i$, and get the corresponding worker $w_{(i)}$;
%
%            %\State initialize $x^1_{\tau_i,w}=0$ for all $\tau_i \in \tau $, $w \in W_i$;
%            %\State $\tau_x:= argmax \left\{ Quality(\tau) : f(\tau_i)=1, \tau_i \in \tau \right\}$;
%            %\State
%            \State select the task assignments matrix $x_1$ which can get the highest task finishing quality, and satisfy $\tau_e<q$ and $TC(x_1)\leq Budget$;
%
%            %\State prune workers that do not meet the limited $Budget$, and get valid workers $W'$;
%
%
%            %\State initialize $x^2_{\tau_i,w}=0$ for all $\tau_i \in \tau $, $w \in W_i$;
%            \For{ select $q$ subtasks $\tau_q$ to be executed}
%            %\State initialize the total traveling cost $\widetilde{c}=0$;
%            \State $\tau:=\tau \backslash \tau_q$;
%            \While {$\tau \neq \emptyset $}
%            \For{ $ \tau_i \in \tau $ }
%            \If{we cannot prune subtask $\tau_i$ by Lemma \ref{prune3}}
%            \State compute $ Quality(\tau_i)^* $;
%            \EndIf
%            \EndFor
%
%            \State $\tau_x:= argmax\left\{ q : \tau_i \in \tau \right\}$;
%            %\If{$ \widetilde{c} + TC(\tau_x) \leq Budget$}
%                %\State set $x^2_{\tau_x, w_{(x)}}=1$;
%                %\State $\widetilde{c}=\widetilde{c}+TC(\tau_x)$
%            %\EndIf
%            \State $\tau:=\tau \backslash \tau_x$;
%
%            \EndWhile
%            \EndFor
%            \State select the task assignment matrix $x_2$ which can get the highest task quality.
%            \State \Return $x$ with the highest task finishing quality, $x \in \left\{x_1,x_2\right\} $;
%        \end{algorithmic}
%        \end{algorithm}
%
%    {\bfseries Pruning Strategies}: The approximation algorithm \ref{single-alg2} first adopts a partial enumeration heuristic, and the time complexity of this process may up to $O(m^q)$. However, according to the properties of $Quality$, it is not efficient to enumerate all sets of up to $q$ subtasks.
%
%        \begin{lemma}
%        \label{prune5}
%        (Quality Pruning) Let $s_1$ and $s_2$ denote the set of executed subtasks of a task $\tau$, $s_1 \subset s_2$. Both executed cases satisfy the limited $Budget$, it's clear that the $Quality$ of $s_2$ is higher than the other one.
%        \end{lemma}
%
%        \begin{lemma}
%        \label{prune6}
%        (Budget Pruning) Let $s_1$ and $s_2$ denote the set of executed subtasks of a task $\tau$, $s_1 \subset s_2$. If the task cost of $s_1$ is larger than the limited $Budget$, the task cost of $s_2$ is also larger than $Budget$.
%        \end{lemma}
%
%        \begin{figure}
%        \centering
%        \includegraphics[height=5.5cm, width=6.5cm]{fig/prune.pdf}
%        \caption{Pruning Strategy}
%        \label{prun}
%        \end{figure}
%        As show in Fig.\ref{prun}, the dotted box denotes the task cost of this set is larger than $Budget$, so adding more subtask into this set does not meet the constraint according to Lemmas \ref{prune6}. While solid box denote the task cost of this set satisfies the $Budget$ constraint, then we do not consider about the subset of this set anymore, as this set has the highest task finishing quality according to Lemmas \ref{prune5}.
%
%        Thus, by utilizing the Lemmas \ref{prune5} and \ref{prune6}, we can prune some sets that can not be the result of the algorithm.
%
%    {\bfseries Time complexity}: We try to present the time complexity of the algorithm \ref{single-alg2}. First, selecting the nearest online worker using R-tree for each time slot, and the time cost is $O(mlogn)$. Then, the time cost of enumerates all sets of up to $q$ subtasks is $O(m^q)$. Thus, for each set that has $q$ subtasks, the algorithm \ref{single-alg2} select the pair with the highest task finishing quality ratio until the limited Budget is reached. Each process is about $O(m^2)$. In summary, the total time complexity of the algorithm \ref{single-alg2} can be given by $O(m^{q+2}+m^q+mlogn)$.


==> response.tex <==
\clearpage
\twocolumn[
    \begin{center}
        \huge
        Response Letter
    \end{center}
    ]

We would like to thank reviewers for their insightful and valuable comments. We have significantly revised the paper according to the comments. The responses to each review comment are listed as below.

\subsection{Response to Reviewer \#1}
{\bf O1.} Thanks for your comments. We improve the presentation by giving more intuitions. In particular, we explain more on round complexity and partitioning quality in Section~\ref{subsec:analysis}. We also improve the presentation on the relation between partitioning quality and distributed graph computing in Section~\ref{subsec:partition-quality}.

{\bf O2.} Thanks. We add the experiment on partitioning quality w.r.t. graph sizes, from $10K$ to $60M$, as shown in Figure~\ref{ret:sample-graph}.

{\bf O3.} Thanks. The links of source codes of competitors and default parameters are introduced in Section~\ref{sec:exp}. We add the discussion of parameters of batch size, imbalance factor $\tau$, and relative weights, in Section~\ref{subsec:result}, and corresponding results are shown in Figure~\ref{ret:parallel} (b) and Figure~\ref{ret:Analysis}.
%We also analyze the effect of parameters of CLUGP in Section~\ref{sec:exp}.

{\bf O4.} Thanks. We use PUMBA to simulate different networking latencies of docker environments, and discuss it in Section~\ref{subsec:result}. The result is shown in Figure~\ref{ret:pagerank} (c).

{\bf O5.}
Thanks. The intra-node parallelization will not affect the partitioning quality. As Figure~\ref{fig:algorithm} (d) shows, clusters are split into batches, so the number of tasks only depends on the batch size and is independent to the number of threads.
So, the intra-node parallelization only affects the algorithm running time, as shown in Figure~\ref{ret:parallel} (a). Also, we show how the batch size affects the partition quality in Figure~\ref{ret:parallel} (b).

{\bf R1.} Thanks. We conduct experiments to observe the trend of replication factor with varied relative weights. The result is shown in Figure~\ref{ret:Analysis} (b). We add corresponding discussion in Section~\ref{subsec:result}.

\subsection{Response to Reviewer \#2}
{\bf O1.} Thanks for your comments.
In our paper, the first step of the framework, steaming clustering, is claimed to be modularity-based. It is for two reasons: 1) our paper is about the study of web graphs, which are with high modularity, as shown in Table~\ref{tab:modularity}; 2) the modularity is a quality metric in graph clustering, which is used for verifying the effectiveness of clustering optimization. In the revised version, we have: 1) improved the presentation by emphasizing the connections with modularity when presenting streaming clustering;
2) used modularity to show the effectiveness our proposed splitting operation, where the graph modularity can be proved to be improved (Theorem~\ref{th:modulairt-based}).

\subsection{Response to Reviewer \#3}
{\bf O1.} %We would like to point out that the scope of the manuscript is on web graphs instead of social graphs (datasets of \cite{petroni2015hdrf}). The first step of the framework is on clustering which is modularity-based and web graphs often have high modularity values, as shown in Table~\ref{tab:modularity}, showing a good match between data and methodologies. The social graphs, however, do not have high modularity of values, as shown in Table~\ref{tab:modularity-social}.
Thanks for your comments. We have added experiments on social graphs, in Figure~\ref{ret:twitter}. Although the replication factor of CLUGP is slightly higher than HDRF,
the total task runtime cost, including graph partitioning and distributed algorithm execution, of CLUGP is lower, because of the impregnable lead of CLUGP in partitioning efficiency.
%the partitioning time cost of CLUGP is much lower than HDRF.
Even so, we feel it is not ready to say CLUGP is better than HDRF on social graphs, because its replication factor is still slightly higher. So, for this paper, we would like to limit the scope to web graphs, as what we claim in the paper. We have added corresponding discussions and will study the optimization on social graphs in the future.

{\bf O2.} Thanks. We have improved the presentation of partitioning metrics in Section~\ref{subsec:setup}.
We use two commonly accepted metrics, replication factor and relative load balance, to measure the partitioning quality, as emphasized in Section~\ref{subsec:partition-quality}.

%Furthermore, we also present the significance of the partitioning metrics in Section~\ref{subsec:partition-quality}.

{\bf O3.} Thanks. We set the imbalance factor $\tau$ to $1.0$, and update the results on replication factor in Figure~\ref{ret:quality} (a-d). The results are mostly the same as before.
We also observe the trend of replication factor by varying the imbalance factor, in Figure~\ref{ret:Analysis} (a). The result shows the effect of imbalance factor is marginal.

\subsection{Response to Reviewer \#4}
{\bf O1.} Thanks for your comments.
We have added experiments on social graphs, in Figure~\ref{ret:twitter}. Although the replication factor of CLUGP is slightly higher than HDRF,
the total task runtime cost, including graph partitioning and distributed algorithm execution, of CLUGP is lower, because of the impregnable lead of CLUGP in partitioning efficiency.
%the partitioning time cost of CLUGP is much lower than HDRF.
Even so, we feel it is not ready to say CLUGP is better than HDRF on social graphs, because its replication factor is still slightly higher. So, for this paper, we would like to limit the scope to web graphs, as what we claim in the paper. We have added corresponding discussions and will study the optimization on social graphs in the future.


%Thanks for your comments. We would like to point out that the scope of the manuscript is on web graphs instead of social graphs (datasets of \cite{petroni2015hdrf}). The first step of the framework is on clustering which is modularity-based and web graphs often have high modularity values, as shown in Table~\ref{tab:modularity}, showing a good match between data and methodologies. The social graphs, however, do not have high modularity of values, as shown in Table~\ref{tab:modularity-social}. We also do the experiments on social graph, as shown in Figure~\ref{ret:twitter}. Although the replication factor of CLUGP is slightly higher than HDRF, the partitioning time cost of CLUGP is much lower than HDRF. Even so, we feel it is not ready to say CLUGP is better than HDRF on social graphs, because it does not give a lower replication factor. So, for this paper, we would like to limit the scope to web graphs, and we will study the extension of the framework to social graphs in our future work.

{\bf O2.} Thanks. We have added Section~\ref{sec:related} to discuss details of related works and distinguish our work from them.

{\bf O3.} Thanks. We would like to argue that the proposed splitting operation is simple yet effective. If adopting the idea in \cite{gonzalez2012powergraph}, i.e., randomly assigning cutting edges to different partitions, the benefits of vertex-cut partitioning (reducing vertex replicas) would not be well exploited. In other words, the idea of \cite{gonzalez2012powergraph} only forcedly transforms edge-cut partitions to vertex-cut partitions, without addressing the difference between the targets of edge- and vertex-cut partitioning.

%The detailed discussion is shown in Section~\ref{subsec:cluframework}. A straightforward way of transforming vertex partitioning to edge partitioning is to randomly assign cut edges to different partitions~\cite{gonzalez2012powergraph}. Actually, the methods~\cite{gonzalez2012powergraph} does not consider the characteristic of edge partitioning (reducing vertex replicas), but simply performs conversion after the vertex partitioning is completed. Furthermore, the challenge we face is how to properly apply edge partitioning in the dynamic process of streaming vertex clustering.

%{\bf O3.} We set the imbalance factor $\tau$ to $1.0$, and update the results on replication factor in Figure~\ref{ret:quality} (a-d). The results are mostly the same as before.
%We also observe the trend of replication factor by varying the imbalance factor, in Figure~\ref{ret:ablation} (b). The result shows the effect of imbalance factor is marginal.

{\bf O4.}
Thanks. We set the imbalance factor $\tau$ to $1.0$, and update the results on replication factor in Figure~\ref{ret:quality} (a-d).
The results are mostly the same as before, demonstrating that the replication factor of CLUGP is the lowest.
%Without loss of generality, we set the imbalance factor $\tau=1.0$, which is same as other competitors. The partitioning results are shown in Figure~\ref{ret:quality}.
To further present the effect of partitioning metrics on distributed system performance, we divided the total task running time into computing time and communication time, as shown in Figure~\ref{ret:pagerank} (b-c).
In all testings, CLUGP has the lowest computing time and communication time. We have incorporated above discussions to the manuscript, in Section~\ref{sec:exp}. 
